Characterization of uncertainties in electron-argon collision cross sections

The predictive capability of a plasma discharge model depends on accurate representations of electron-impact collision cross sections, which determine the key reaction rates and transport properties of the plasma. Although many cross sections have been identified through experiments and quantum mechanical simulations, their uncertainties are not well-investigated. We characterize the uncertainties in electron-argon collision cross sections using a Bayesian framework. Six collision processes -- elastic momentum transfer, ionization, and four excitations -- are characterized with semi-empirical models, whose parametric uncertainties effectively capture the features important to the macroscopic properties of the plasma, namely transport properties and chemical reaction rates. The method is designed to capture the effects of systematic errors that lead to large discrepancies between some data sets. Specifically, for the purposes of Bayesian inference, each of the parametric cross section models is augmented with a Gaussian process representing systematic measurement errors as well as model inadequacies in the parametric form. The results show that the method is able to capture scatter in the data between the electron-beam experiments and ab-initio quantum simulations. The calibrated cross section models are further validated against measurements from swarm-parameter experiments.

==> packages.tex <==
\usepackage{amsmath}
\usepackage{iopams}  
\usepackage{amssymb,amsthm}
\usepackage{bbm}
%\usepackage[dvipsnames]{xcolor}

\usepackage[numbers,sort&compress]{natbib}
\bibliographystyle{iopart-num}
\newcommand{\newblock}{}

\usepackage{hyperref}

\usepackage[disable]{todonotes}

\usepackage{multirow, multicol}
\usepackage{makecell}
\usepackage{csquotes}

\usepackage{tikz}
\usetikzlibrary{positioning}
\usepackage{pgfplotstable}
\usepackage{pgfplots}
\pgfplotsset{compat=1.10}
\usepgfplotslibrary{groupplots,fillbetween}

\definecolor{burntorange}{RGB}{191,87,0}

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF CFONT PREAMBLE %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue} \sf #1}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red} \scriptsize #1}} %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
\providecommand{\DIFmodbegin}{} %DIF PREAMBLE
\providecommand{\DIFmodend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF COLORLISTINGS PREAMBLE %DIF PREAMBLE
\RequirePackage{listings} %DIF PREAMBLE
\RequirePackage{color} %DIF PREAMBLE
\lstdefinelanguage{DIFcode}{ %DIF PREAMBLE
%DIF DIFCODE_CFONT %DIF PREAMBLE
  moredelim=[il][\color{red}\scriptsize]{\%DIF\ <\ }, %DIF PREAMBLE
  moredelim=[il][\color{blue}\sffamily]{\%DIF\ >\ } %DIF PREAMBLE
} %DIF PREAMBLE
\lstdefinestyle{DIFverbatimstyle}{ %DIF PREAMBLE
	language=DIFcode, %DIF PREAMBLE
	basicstyle=\ttfamily, %DIF PREAMBLE
	columns=fullflexible, %DIF PREAMBLE
	keepspaces=true %DIF PREAMBLE
} %DIF PREAMBLE
\lstnewenvironment{DIFverbatim}{\lstset{style=DIFverbatimstyle}}{} %DIF PREAMBLE
\lstnewenvironment{DIFverbatim*}{\lstset{style=DIFverbatimstyle,showspaces=true}}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

==> sections-orig/abstract.tex <==
The predictive capability of a plasma discharge model depends on accurate representations of electron-impact collision cross sections,
which determine the key reaction rates and transport properties of the plasma.
Although many cross sections have been identified through experiments and quantum mechanical simulations,
their uncertainties are not well-investigated.
%
We characterize the uncertainties in electron-argon collision
cross sections using a Bayesian framework.  Six collision
processes---elastic momentum transfer, ionization, and four
excitations---are characterized with semi-empirical models, whose
parametric uncertainties effectively capture the features important to
the macroscopic properties of the plasma, namely
transport properties and chemical reaction rates.  The method is
designed to capture the effects of systematic errors that lead to
large discrepancies between some data sets.  Specifically, for the
purposes of Bayesian inference, each of the parametric cross section models
is augmented with a Gaussian process representing systematic
measurement errors as well as model inadequacies in the parametric
form.  The results show that the method is able to capture scatter in the data between the
electron-beam experiments and \textit{ab-initio} quantum
simulations.  The calibrated cross section models are further
validated against measurements from swarm-parameter experiments.
%
% TAO: Rewrote the last few sentences of the abstract.  The original is retained below for reference.
%
%The likelihood is evaluated against the electron-beam experiments and \textit{ab-initio} simulations.
%Due to their own inferences or estimations, these measurement datasets have a large discrepancy that cannot be explained by their own reported accuracies,
%and the likelihood model only with the goodness-of-fit can lead to an unrealistic and biased conclusion.
%Our likelihood model reflects this systematic error, as well as the model inadequacy, with a Gaussian-process model.
%The resulting uncertainty well-captures the scattering among the measurement datasets,
%and is further validated against the swarm-parameter experiments,
%via a 0D-Boltzmann analysis (\texttt{BOLSIG}).

==> sections-orig/bayes.tex <==
\section{Uncertainty quantification via Bayesian inference}\label{sec:bayes}

\subsection{Overall framework}
We represent the uncertainty of a cross section $\sigma(\epsilon)$
with the parametric uncertainty of the corresponding semi-empirical model $f(\epsilon;\vec{A})$ calibrated with the given measurement data $\mathcal{M}$.  Specifically, this information is encoded in the probability distribution $P[\vA \vert\cM]$, which is the distribution for the model parameters conditioned on the observations in $\mathcal{M}$.
As shown in Figure~\ref{fig:crs-curation},
each cross section has corresponding measurement data $\mathcal{M}$ composed of multiple datasets,
\begin{subequations}
\begin{equation}
\cM = \{\cM_1, \cM_2, \ldots, \cM_M\}.
\end{equation}
Each dataset $\cM_m$ consists of data points $(\veps_m, \vsig_m)$ and reported measurement uncertainties $\Dvsig_m$,
\begin{equation}
\cM_m = (\veps_m, \vsig_m, \Dvsig_m),
\quad
m = 1, \cdots, M,
\end{equation}
where $\veps_m, \vsig_m, \Dvsig_m \in \rR^{N_m}$, and $N_m$ denotes the number of data points in the dataset $\cM_m$.
\end{subequations}
\par
According to the Bayes' law, the desired parametric uncertainty $P[\vA\vert\cM]$ is
\begin{equation}\label{eq:bayes0}
\underbrace{P[\vA\vert\cM]}_{\text{posterior}} \propto \underbrace{P[\cM \vert \vA]}_{\text{likelihood}}\; \underbrace{P[\vA]}_{\text{prior}}.
\end{equation}
The prior distribution $P[\vA]$ is a probabilistic representation of any information about the parameters $\vA$ that is available separate from the data $\mathcal{M}$.
For given parameters $\vA$, the likelihood $P[\cM \vert \vA]$ is the probability distribution for the measurements conditiond on $\vA$.
For given data $\mathcal{M}$, the likelihood is a function of $\vA$
that encodes the logic that
values for $\vA$ that make the observed values of the measurements a
more probable outcome of the model should be favored over parameter
values that make the observations less likely, all other things being
equal.
%\todo{SWC: I'm somewhat confused by this sentence. Is this providing the frequentist's viewpoint?}
% TAO: No, nothing frequentist, just trying to give intuition for the likelihood.
%
%In general, the absolute magnitude of the posterior $P[\vA \vert \cM]$ is not important,
%since it is constrained by the normalization condition
%\begin{equation}
%\int P[\vA \vert \cM]\; d\vA = 1.
%\end{equation}
\par
The formulation of the right-hand side of (\ref{eq:bayes0}) is not unique.  That is, in most complicated problems at least, there are not clearly establishable, true distributions for the prior and likelihood.  Instead, these distributions are mathematical models that represent a given state of information.  Different models could reflect, for instance, different interpretations of the data or different hypotheses about the nature of the important uncertainties.  Thus, the formulation can differ depending on what uncertain factors are considered and how they are modeled.

To illustrate this fact and the implications of different choices, three likelihood formulations are introduced below.
In Section~\ref{subsec:wrong-bayes-1}, we introduce the simplest likelihood formulation that only considers the measurement uncertainty.
An alternative formulation is provided in Section~\ref{subsec:wrong-bayes-2},
where the systematic error is also considered as a type of parametric uncertainty.
Lastly in Section~\ref{subsec:gp-bayes},
we propose a likelihood formulation where the systematic error is not absorbed into the cross section model parameters.
It will be shown in Section~\ref{sec:result}
that this approach is most appropriate in the present setting,
%the last formulation is deemed properly reflecting the problem statement,
while the first two can lead to misleading conclusions.

\subsection{A likelihood formulation with the measurement error only}\label{subsec:wrong-bayes-1}
We first consider the reported measurement errors as the only uncertainty.
With the assumption that each dataset is obtained independently,
the resulting likelihood of the overall data $\cM$ is
\begin{equation}\label{eq:wrong-bayes1-total-likelihood1}
P_1\left[\cM \big| \vA \right] = \prod_{m=1}^M P_1\left[\cM_m \big| \vA \right],
\end{equation}
where a subscript for $P$ is used to discern different likelihoods.
For the $n$-th data point $(\epsilon_{m,n}, \sigma_{m,n})$ in a dataset $\cM_m$,
we consider a \textit{measurement} model with a multiplicative measurement error $\delta\sigma_{m,n}$,
\begin{equation}\label{eq:wrong-bayes1-measurement-model}
\sigma_{m,n} = f(\epsilon_{m,n}; \vA) \times \delta\sigma_{m,n},
\end{equation}
so that
%so instead of (\ref{eq:log-sigma-model1}),
\begin{equation}\label{eq:wrong-bayes1-statement}
\log\sigma_{m,n} = \log f(\epsilon_{m,n}; \vA) + \log\delta\sigma_{m,n}.
\end{equation}
%We keep the original expression for the posterior (\ref{eq:bayes0}),
%with the priors (\ref{eq:prior-el}--\ref{eq:prior-resonance}).
We assume the logarithm of the measurement error $\log\dvsig_m$ follows an independent Gaussian distribution based on the reported relative error,
\begin{equation}\label{eq:measurement-error}
P(\log\dvsig_m) = \cN\left[ 0, \mathrm{diag}\left(\log^2(1 + \frac{\Dvsig_m}{\vsig_m} )\right) \right],
\end{equation}
where all arithmetic operations between vectors are element-wise.
This logarithmic scale model is justified by the fact that
the majority of the measurement data report their accuracy in terms of the relative error $\Dvsig / \vsig$.
While the BSR dataset does not report the accuracy of the dataset,
we imposed a $10\%$ relative error based on its credibility as described in Section~\ref{subsec:electron-beam}.
With the probability model (\ref{eq:measurement-error}),
the likelihood of a dataset $\cM_m$ based on (\ref{eq:wrong-bayes1-statement}) is
\begin{equation}\label{eq:wrong-bayes1-total-likelihood2}
P_1\left[ \cM_m \big| \vA \right] = \cN\left[ \log f(\veps_m; \vA), \mathrm{diag}\left( \log^2 (1 + \frac{\Dvsig_m}{\vsig_m}) \right) \right].
\end{equation}
\par
%\todo[inline]{Might have to revisit how we impose the priors..}
The prior $P(\vA)$ is imposed based on any prior knowledge about the collision cross section models.
For the total ionization cross section, there is no reported value for $\vA_i$, and therefore the uniform prior $P(\vA_i) = 1$ is imposed.
For the elastic momentum-transfer collision,
a Gaussian probability is imposed on $\vA_{MERT}$ based on the literature value from Haddad and O'Malley~\cite{Haddad1982}
with $50\%$ relative standard deviation,
\begin{equation}\label{eq:prior-el}
P(\vA_{el}) = P(\vA_{MERT}) = \cN\left[\vA_{MERT, ref}, \mathrm{diag}\left((0.5\vA_{MERT, ref})^2\right) \right],
\end{equation}
with $\vA_{MERT, ref} = \{-1.488, 65.4, -84.3, 0.983\}$.
For the metastable-level excitation cross sections,
a Gaussian probability is imposed on $\vA_{me}$ based on the literature values from Bretagne \textit{et al.}~\cite{Bretagne1986}
with $100\%$ relative standard deviation,
\begin{equation}
P(\vA_{me}) = \cN\left[ \vA_{me, ref}, \mathrm{diag}\left(\vA_{me, ref}^2\right) \right],
\end{equation}
with $\vA_{1s5} = \{51.2, 2.0\}$ and $\vA_{1s3} = \{10.4, 2.0\}$.
For the resonance-level excitation cross sections,
a Gaussian probability is imposed on $F_{0,r}$ based on the literature values from Bretagne \textit{et al.}~\cite{Bretagne1986}
with $100\%$ relative standard deviation,
\begin{equation}\label{eq:prior-resonance}
P(\vA_{r}) = P(F_{0,r}) = \cN\left[ F_{0,r,ref}, F_{0,r,ref}^2 \right],
\end{equation}
with $F_{0, 1s4, ref} = 0.061$ and $F_{0, 1s2, ref} = 0.254$.
\par
To examine how the data impacts the uncertainty of $\vA$ under this formulation,
we consider two cases.  In the first, each data set is used individually, so that the posterior is given by
\begin{equation}\label{eq:wrong-bayes1-indiv}
P_1\left[ \vA \big| \cM_m \right] \propto P_1\left[ \cM_m \big| \vA \right] P(\vA),
\end{equation}
with the individual likelihood (\ref{eq:wrong-bayes1-total-likelihood2}) and the priors (\ref{eq:prior-el}--\ref{eq:prior-resonance}).
In the second, all the data are used simultaneously, so that
\begin{equation}\label{eq:wrong-bayes1-total}
P_1\left[ \vA \big| \cM \right] \propto \prod_{m=1}^M P_1\left[ \cM_m \big| \vA \right] P(\vA),
\end{equation}
with the overall likelihood (\ref{eq:wrong-bayes1-total-likelihood1}) and the same priors (\ref{eq:prior-el}--\ref{eq:prior-resonance}).

\subsection{All systematic error represented as the parametric uncertainty}\label{subsec:wrong-bayes-2}
In Section~\ref{sec:curation}, we note that the measurement data $\cM$ exhibits a large scattering among the datasets $\cM_m$
which is much larger than their reported observation errors $\Dvsig_m$.
%Also, the employed semi-empirical models do not capture all the features at all scales,
%thus a model-form error is involved in calibrating the uncertainty for $\vA$.
This systematic error may not be negligible and thus should be accounted for in the probabilistic model using in the inference process.
One approach is to model the systematic error as an additional parametric uncertainty,
%so instead of having a disturbance on the cross section itself as for $\delta f$ in (\ref{eq:log-sigma-model1}),
so each dataset $\cM_m$ may have a disturbance $\delta \vA_m$ in its parameter value,
\begin{equation}\label{eq:A-model1}
\vA_m = \vA + \delta \vA_m.
\end{equation}
This disturbance may be modeled to follow a joint Gaussian distribution over the parameter $\vA$-space
with a covariance,
\begin{equation}\label{eq:dA-model}
P_2\left[ \delta\vA_m \big| \vtheta \right] = \cN\left[ \vec{0}, \Sigma(\vtheta) \right],
\end{equation}
where, considering the symmetry of the covariance, $\vtheta$ corresponds to all the entries of the upper-triangular part of $\Sigma$.
Aside from the true $\vA$, several additional variables are considered uncertain in this viewpoint:
$\{\vA_m\}_{m=1}^M$ the realizations of $\vA$ for all datasets and the model parameter $\vtheta$.
The Bayes' law (\ref{eq:bayes0}) then should reflect all the uncertain variables,
having the resulting joint posterior,
\begin{equation}\label{eq:wrong-bayes2-joint-posterior}
\begin{split}
P_2\left[ \vA, \vtheta, \{\vA_m\}_{m=1}^M \big| \cM \right]
&\propto
P_2\left[ \cM, \{\vA_m\}_{m=1}^M \big| \vA, \vtheta \right]
\;
P[\vA]\; P_2[\vtheta]\\
&\propto
\prod_{m=1}^M P_2\left[ \cM_m \big| \vA_m, \vA, \vtheta \right] \; P_2\left[ \vA_m \big| \vA, \vtheta \right]
\;
P[\vA]\; P_2[\vtheta].
\end{split}
\end{equation}
For the cross section model parameter $\vA$ as our primary interest,
we consider all possibilities for $\{\vA_m\}_{m=1}^M$ and $\vtheta$ and thus marginalize $P_2\left[ \vA, \vtheta, \{\vA_m\}_{m=1}^M \big| \cM \right]$ over $\{\vA_m\}_{m=1}^M$ and $\vtheta$,
\begin{equation}\label{eq:wrong-bayes2}
P_2\left[ \vA \big| \cM \right]
= \int P_2\left[ \vA, \vtheta, \{\vA_m\}_{m=1}^M \big| \cM \right]\;d\vtheta d\vA_1 \cdots d\vA_M.
\end{equation}
%which is a refined description of (\ref{eq:bayes0}).
\par
With (\ref{eq:A-model1}) and (\ref{eq:dA-model}), the likelihood for $\vA_m$ is
\begin{equation}
P_2\left[ \vA_m \big| \vA, \vtheta \right] = \cN\left[ \vA, \Sigma(\vtheta) \right].
\end{equation}
When the parameter is realized as $\vA_m$ in the measurement $m$, the likelihood of the dataset $\cM_m$ is
\begin{equation}\label{eq:wrong-bayes2-likelihood}
P_2\left[ \cM_m \big| \vA_m, \vA, \vtheta \right] = \cN\left[ \log f(\veps_m; \vA_m), \mathrm{diag}\left( \log^2 (1 + \frac{\Dvsig_m}{\vsig_m}) \right) \right],
\end{equation}
which is similar to (\ref{eq:wrong-bayes1-total-likelihood2}) but the expected cross section is based on $\vA_m$.
\par
The same priors (\ref{eq:prior-el}--\ref{eq:prior-resonance}) are used for $P[\vA]$.
For the systematic error model parameter $\Sigma(\vtheta)$,
there is little information available to inform the probablilty for $\vtheta$,
and we can only expect that the corresponding variances would not be extremely small or large
compared to the parameter value itself.
% \todo{TAO: Extremely large or small relative to what?}
Thus we assume the corresponding variances to be uniform on the logarithmic scale,
\begin{subequations}\label{eq:wrong-bayes2-hyper-prior}
\begin{equation}
P_2[\vtheta] = \prod_{d=1}^{\mathrm{dim}(\Sigma)}P_2\left[V_d(\vtheta)\right]
\end{equation}
\begin{equation}
P_2\left[V_d(\vtheta)\right] = 
\begin{cases}
\frac{1}{V_d(\log V_{d, max} - \log V_{d, min})}
& V_d \in [V_{d, min}, V_{d, max}]\\
0 & \text{otherwise,}
\end{cases}
\end{equation}
\end{subequations}
with $V_d(\vtheta)$ the variance along the $d$-th principal axis of $\Sigma(\vtheta)$
% \todo{TAO: I don't understand how $\Sigma$ is constructed if you only have a distribution on the singular values.\\
% SWC: It's the other way around--- $V_d$ is evaluated based on $\Sigma$. This way we do not restrict correlation between parameters.}
and $V_{d, min} = 10^{-2}$ and $V_{d, max} = 10^{1}$.
In actual evaluation, $V_d$ is determined as the $d$-th singular value of $\Sigma(\vtheta)$ given the parameter $\vtheta$.
The posterior (\ref{eq:wrong-bayes2}) is then evaluated with (\ref{eq:wrong-bayes2-joint-posterior}), (\ref{eq:wrong-bayes2-likelihood}), (\ref{eq:prior-el}--\ref{eq:prior-resonance}) and (\ref{eq:wrong-bayes2-hyper-prior}).
\par
%Compared to Section~\ref{subsec:gp-bayes},
This description is predicated upon a strong assumption that the
model-form error is negligible and that systematic differences between
the experiments are due to each separate experiment realizing
different values of the semi-empirical model parameters.
It shall be seen in Section~\ref{sec:result} how this assumption impacts the results for $\vA$.

\subsection{A probabilistic description with a model for the systematic error}\label{subsec:gp-bayes}
%\todo[inline]{Debating whether top-down or bottom-up description would be better..}

%The strong assumption in Section~\ref
%Unlike the viewpoint in Section~\ref{subsec:wrong-bayes-2},
%Our viewpoint 
%the systematic errors exhibited in the measurement $\cM$ may not be well characterized with 
%
%In Section~\ref{sec:curation}, we note that the measurement data $\cM$ exhibits a large scattering among the datasets $\cM_m$
%which is much larger than their reported observation errors $\Dvsig_m$.

While the measurement data $\cM$ exhibits a systematic error among the datasets $\cM_m$,
the employed semi-empirical models also do not necessarily capture all the features at all scales.
For example, the BSR excitation cross sections in Figure~\ref{fig:crs-curation}~(c--f) exhibits
small-scale variations near $\epsilon-\epsilon_0 \sim 1 eV$,
which cannot be represented at all by the model forms introduced in Section~\ref{sec:model}.
Thus, in addition to the systematic errors in the data, a model-form error is present.
The combined effect of the systematic data errors and the model inadequacies is denoted by $\delta f$ here.
Specifically, similar to (\ref{eq:wrong-bayes1-measurement-model}),
we consider a measurement model for the $n$-th data point $(\epsilon_{m,n}, \sigma_{m,n})$ in a dataset $\cM_m$,
where $\delta f$, which depends on additional parameters denoted $\vtheta$, appears as an additional multiplicative factor,
\begin{equation}
\sigma_{m,n} = f(\epsilon_{m,n}; \vA) \times \delta f(\epsilon_{m,n}; \vtheta) \times \delta\sigma_{m,n},
\end{equation}
which implies that
\begin{equation}\label{eq:log-sigma-model1}
\log\sigma_{m,n} = \log f(\epsilon_{m,n}; \vA) + \log\delta f(\epsilon_{m,n}; \vtheta) + \log\delta\sigma_{m,n}.
\end{equation}
\par
The resulting joint posterior analogous to (\ref{eq:wrong-bayes2-joint-posterior}) is
\begin{equation}\label{eq:gp-bayes-joint-post}
P_3\left[ \vA, \vtheta \big| \cM \right] \propto P_3\left[\cM \big| \vA, \vtheta \right]\;P\left[\vA \right]\;P_3\left[\vtheta \right],
\end{equation}
where the parameters $\vA$ and $\vtheta$ are taken to be independent in the prior.
Similar to (\ref{eq:wrong-bayes2}),
we consider all possibilities for $\vtheta$ and thus marginalize $P\left[ \vA, \vtheta \big| \cM \right]$ over $\vtheta$,
\begin{equation}\label{eq:gp-bayes-margin-post}
P_3\left[ \vA \big| \cM \right] \propto \int P_3\left[\cM \big| \vA, \vtheta \right]\;P\left[\vA \right]\;P_3\left[\vtheta \right]\; d\vtheta.
\end{equation}
\par
With the assumption that each dataset is obtained independently,
the resulting likelihood of the overall data $\cM$ is
\begin{equation}\label{eq:gp-bayes-total-likelihood}
P_3\left[\cM \big| \vA, \vtheta \right] = \prod_{m=1}^M P_3\left[\cM_m \big| \vA, \vtheta \right],
\end{equation}
where $P_3\left[\cM_m \big| \vA, \vtheta \right]$ will be determined from (\ref{eq:log-sigma-model1})
with the uncertainty models for $\log\dvsig_m$ and $\delta f(\vec{\epsilon}_m;\vA)$.
\par
While the same model (\ref{eq:measurement-error}) is used for the measurement uncertainty $\log\dvsig_m$,
modeling $\delta f(\epsilon; \vtheta)$ requires further development.
Unlike the cross section itself,
it is difficult to model the discrepancy as a simple analytical function as $f(\epsilon;\vA)$.
As described in Section~\ref{sec:curation},
there are many potential factors involved in the discrepancy among datasets, each of which is hard to quantify.
This is further aggravated by the fact
that we have no knowledge to separate the model inadequacy from the systematic error so that they may be modeled individually.
\par
In this situation,
Gaussian processes (GP) provide a flexible probabilistic framework for representing the observed combined effects of these errors.
%where any finite number of samples from $\epsilon$-space follow a joint Gaussian distribution
Specifically, for a given $\vtheta$ and a dataset $\cM_m$, we model
$\log\delta f(\veps_m)$ as a Gassian random function with zero mean and covariance $\bK(\veps_m, \veps_m; \vtheta)\in\rR^{N_m\times N_m}$,
\begin{equation}\label{eq:gp-systematic-error}
P_3\left[ \log\delta f(\veps_m) \;\big|\; \vtheta \right] = \cN\left[ \vec{0}, \bK(\veps_m, \veps_m; \vtheta)\right].
\end{equation}
Each entry of the covariance matrix is determined by the covariance kernel $k$,
\begin{equation}
\bK(\veps_m, \veps_m; \vtheta)_{ij} = k( d_{m, ij} ; \vtheta),
\end{equation}
where $d_{m, ij}$ the distance between two data points $\epsilon_{m,i}$ and $\epsilon_{m,j}$ is determined in the logarithmic scale, based on the scaling behavior of each collision cross section.
For the elastic cross section,
\begin{subequations}
\begin{equation}
d_{m, ij} = \vert \log\epsilon_{m,i} - \log\epsilon_{m,j} \vert,
\end{equation}
and for the other collisions with threshold energy $\epsilon_0$,
\begin{equation}
d_{m, ij} = \vert \log(\epsilon_{m,i} - \epsilon_0) - \log(\epsilon_{m,j} - \epsilon_0) \vert.
\end{equation}
\end{subequations}
The widely used Mat\'{e}rn kernel is used for $k(d; \vtheta)$ with model parameters $\vtheta = \{V_{\theta}, d_{\theta}\}$,
\begin{equation}
k(d; \vtheta) = V_{\theta}\frac{2^{1-\nu}}{\Gamma(\nu)}\left( \sqrt{2\nu}\frac{d}{d_{\theta}} \right)^{\nu}K_{\nu}\left( \sqrt{2\nu}\frac{d}{d_{\theta}} \right),
\end{equation}
where $\Gamma$ is the gamma function, $K_\nu$ is the modified Bessel function of the second kind, and $\nu = 1.5$.
$V_{\theta}$ and $d_{\theta}$ are the main parameters of the Mat\'{e}rn kernel that represent the variance and correlation scale, respectively.
\par
With the probability models (\ref{eq:gp-systematic-error}) and (\ref{eq:measurement-error}),
the likelihood of a dataset $\cM_m$ based on (\ref{eq:log-sigma-model1}) is
\begin{equation}\label{eq:gp-bayes-indiv-likelihood}
\begin{split}
P_3\left[\cM_m \big| \vA, \vtheta \right] &= P_3\left[\log\vsig_m \big| \vA, \vtheta \right]\\
&= \cN\left[ \log\delta f(\veps_m;\vA), \bK(\veps_m, \veps_m; \vtheta) + \mathrm{diag}\left( \log^2 (1 + \frac{\Dvsig_m}{\vsig_m} ) \right) \right].
\end{split}
\end{equation}
%This completes the likelihood (\ref{eq:gp-bayes-total-likelihood}) which is evaluated for (\ref{eq:gp-bayes-joint-post}) and (\ref{eq:gp-bayes-margin-post}).
\par
The same priors (\ref{eq:prior-el}--\ref{eq:prior-resonance}) are used for $P[\vA]$.
Analogous to (\ref{eq:wrong-bayes2-hyper-prior}), for the prior $P_3[\vtheta]$,
we assume $V_{\theta}$ to be uniform on the logarithmic scale,
\begin{equation}\label{eq:prior-gp-var}
P_3[\vtheta] = P_3[V_{\theta}] =
\begin{cases}
\frac{1}{V_{\theta}(\log V_{\theta, max} - \log V_{\theta, min})}
& V_{\theta} \in [V_{\theta, min}, V_{\theta, max}]\\
0 & \text{otherwise,}
\end{cases}
\end{equation}
with the range $V_{\theta, min} = 10^{-2}$ and $V_{\theta, max} = 10^{1}$.
\par
The likelihood (\ref{eq:gp-bayes-total-likelihood}), the priors (\ref{eq:prior-el}--\ref{eq:prior-resonance}) and (\ref{eq:prior-gp-var})
then constitutes the posteriors (\ref{eq:gp-bayes-joint-post}) and (\ref{eq:gp-bayes-margin-post}) for all 6 collision cross sections.

%This combined effect thus must be modeled somehow (presumably with some model parameters $\vtheta$), i.e. $\delta f(\epsilon;\vtheta)$,
%, i.e. $\delta f(\epsilon; \vtheta)$, must be correlated in $\epsilon$-space just as for the cross section $\sigma(\epsilon)$ itself,
%and thus also must be modeled somehow (presumably with some model parameters $\vtheta$).
%\par
%Our likelihood formulation reflects the viewpoint that this combined effect of the discrepancies and model inadequacy cannot be neglected
%and thus must be accounted in the cross section measurement.
%This \textit{systematic} error term, i.e. $\delta f(\epsilon; \vtheta)$, must be correlated in $\epsilon$-space just as for the cross section $\sigma(\epsilon)$ itself,
%and thus also must be modeled somehow (presumably with some model parameters $\vtheta$).
%The Bayes' law (\ref{eq:bayes0}) then should reflect the probabilistic description for $\vtheta$,
%\begin{equation}\label{eq:gp-bayes-joint-post}
%P\left[ \vA, \vtheta \big| \cM \right] \propto P\left[\cM \big| \vA, \vtheta \right]\;P\left[\vA, \vtheta \right].
%\end{equation}
%For the cross section model parameter $\vA$ as our primary interest,
%we consider all possibilities for $\vtheta$ and thus marginalize $P\left[ \vA, \vtheta \big| \cM \right]$ over $\vtheta$,
%\begin{equation}\label{eq:gp-bayes-margin-post}
%P\left[ \vA \big| \cM \right] \propto \int P\left[\cM \big| \vA, \vtheta \right]\;P\left[\vA, \vtheta \right]\; d\vtheta,
%\end{equation}
%which is a refined description of (\ref{eq:bayes0}).
%In practice, (\ref{eq:gp-bayes-joint-post}) is evaluated via Markov-chain Monte-Carlo (MCMC) sampling,
%and the integral in (\ref{eq:gp-bayes-margin-post}) corresponds to simply discarding $\vtheta$ information of the samples,
%without a need of arithmetic operations.

%\par
%We assume the logarithm of the measurement error $\log\dvsig_m$ follows an independent Gaussian distribution based on the reported relative error,
%\begin{equation}\label{eq:measurement-error}
%P(\log\dvsig_m) = \cN\left[ \vec{0}, \log^2\left(1 + \frac{\Dvsig_m}{\vsig_m} \right)\mathbf{I} \right],
%\end{equation}
%with the identity matrix $\mathbf{I} \in \rR^{N_m \times N_m}$.
%The majority of the measurement data in fact reported their accuracy in terms of the relative error $\Dvsig / \vsig$.
%While the BSR dataset does not report the accuracy of the dataset,
%we imposed a $10\%$ relative error based on its credibility as described in Section~\ref{subsec:electron-beam}.
\par



==> sections-orig/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
Cross section uncertainties of 6 $e$-$Ar$ collision processes
are quantified via Bayesian inference.
Each cross section is characterized with a semi-empirical model
that captures essential features for plasma reaction and transport,
so its uncertainty is effectively approximated within a low-dimensional parameter space.
Measurement data for cross section inference are curated either from experiments or \textit{ab initio} calculations,
into two categories: direct cross section measurement and swarm-parameter measurement.
The cross section model parameters are then inferred from the direct cross section data.
The resulting distributions are forward-propagated using the \texttt{BOLSIG+} $0D$ Boltzmann equation solver
and validated against the swarm-parameter measurements.
\par
A key aspect of this process is the modeling of discrepancies between different input datasets.
Observation errors reported in direct cross section data are often notional,
not quantitatively reflecting all systematic errors underlying the experiments.
As a result, the discrepancy among datasets is much larger than the reported observation error each claims.
No detailed knowledge of these errors, upon which to base a model, is
available.  Instead, both a parametric representation and a
Gaussian-process-based model were developed, with the
Gaussian-process-based approach giving better results in the present
cases.
%Small observation error or a large number of data points
%do not necessarily imply small systematic error.
%Also, the semi-empirical model cannot perfectly resolve the true cross section, resulting in a model-form error.
%The combined effect of this systematic error and the model-form inadequacy is effectively modeled with a Gaussian process.
%Gaussian-process (GP) effectively modeled the uncertainty of such systematic error,
%being robust against the number of measurements or their reported accuracies.
%As we do not have any knowledge, all possible GP parameters are considered when identifying parametric uncertainties of cross sections.
%\par
%Our current formulation with the GP model implicitly includes such model inadequacy as well.
%Explicit separation of the model inadequacy and the systematic error will inform us more about our knowledge on each cross section.
%This will require \ldots.
\par
%\todo[inline]{TAO: I think we should add a stronger statement about the utility of the process somewhere in the conclusions.\\
%SWC: tried to add some sentences in this paragraph $\downarrow$.}
The resulting cross section uncertainties quantified by this process
provide rich information for the plasma simulations where these calibrated cross sections are used.
For example, the impact of each collision process on the macroscopic plasma observables can be evaluated via sensitivity analysis.
Furthermore, the uncertainties of collision processes can be forward-propagated through the plasma simulations,
thereby evaluating the credibility of the predictive simulations.
\par
As mentioned in Section~\ref{subsec:swarm-data},
the proposed Bayesian inference framework can be extended to incorporate the swarm-analysis data.
As the swarm parameters are determined by the entire set of collisions,
including them into the Bayesian inference will provide richer information as to the correlations between the collision processes.
Since the measurements are made for the swarm-parameters,
evaluating the posterior will require an additional layer of solving the Boltzmann equation model, other than the cross section models themselves.
A similar challenge of handling systematic errors/model-form inadequacy is expected, particularly for the excitation rate coefficient data.
For example,
there are some expected model-form errors which may contribute to the scattering of the data in Figure~\ref{fig:uncertainty-swarm-ex}.
One might be the approximation for radiative de-excitation processes based on the radiative transition probabilities.
The inherent approximation of \texttt{BOLSIG+} that do not track heavy-species population may also have some contribution to this model-form error.
%Quantifying them as an uncertainty, however, have not been considered as it is beyond the scope of our study.
%
%Swarm-parameter measurements implicitly depend on the set of collisions as a whole through the electron energy distribution.
%Although in our study such implicit dependency limited their use only to validation,
%a similar Bayesian framework can be applied to further reflect our knowledge and reduce the uncertainties in cross sections.
%Fortunately, for swarm-parameter measurement, discrepancy among the datasets is much smaller than that for direct cross section measurements.
%The question will be rather how the model-form uncertainties,
%from each cross section to the Boltzmann equation model,
%can be properly factored out and evaluated.


==> sections-orig/curation.tex <==
\section{Cross section measurement datasets}\label{sec:curation}
The available data are split into two subsets: one consisting of
electron-beam experiments and \textit{ab initio} simulation results,
which is used for calibration, and a second consisting of swarm
experiment measurements, which is used for validation.  The
specific data sources as well as relevant features of the data are
described for each of these subsets in
Sections~\ref{subsec:electron-beam} and~\ref{subsec:swarm-data}.

%\todo[inline]{Split each section into two subsections, one for data curation and the other for how to use it.}
\subsection{Electron-beam experiments and \textit{ab initio} calculations}\label{subsec:electron-beam}

\subsubsection{Data characterization}
\begin{table}[tbp]
\centering
\begin{tabular}{|c|c|c|}
\hline
Collision process & Author & Energy range $\epsilon$ ($eV$) \\
\hline
\multirow{5}{8em}{Elastic momentum-transfer, $\sigma_{el}(\epsilon)$} & Zatsarinny \& Bartschat (BSR), 2013~\cite{Pitchford2013, Zatsarinny2013} & $10^{-3}$--$300$\\\cline{2-3}
                                                                                                                & Srivastava \textit{et al.}, 1981~\cite{Srivastava1981} & 3--100\\\cline{2-3}
                                                                                                                & Gibson \textit{et al.}, 1996~\cite{Gibson1996} & 1--10\\\cline{2-3}
                                                                                                                & Panajotovic \textit{et al.}, 1997~\cite{Panajotovic1997} & 10--100 \\\cline{2-3}
                                                                                                                & Mielewska \textit{et al.}, 2004~\cite{Mielewska2004} & 5--10 \\
\hline
\multirow{3}{8em}{Direct ionization ($Ar^+$), $\sigma_{ion}(\epsilon)$} & Rapp \& Englander-Golden, 1965~\cite{Rapp1965} & Threshold--$10^3$ \\\cline{2-3}
								 & Wetzel \textit{et al.}, 1987~\cite{Wetzel1987} & Threshold--200 \\\cline{2-3}
								 & Straub \textit{et al.}, 1995~\cite{Straub1995} & Threshold--$10^3$ \\
\hline
\multirow{6}{8em}{Direct excitation, $\sigma_{ex}(\epsilon)$} & Zatsarinny \& Bartschat (BSR), 2013~\cite{Pitchford2013, Zatsarinny2013} & Threshold--$300$\\\cline{2-3}
                                                                    & Chutjian \& Cartwright, 1981~\cite{Chutjian1981} ($1s_5$--$1s_2$) & Threshold--100 \\\cline{2-3}
    								 & Li \textit{et al.}~\cite{Li1988} ($1s_4$, $1s_2$) & 400, 500 \\\cline{2-3}
    								 & Schappe \textit{et al.}~\cite{Schappe1994} ($1s_5$, $1s_3$) & Threshold--100 \\\cline{2-3}
%    								 & Tsurubuchi \textit{et al.}~\cite{Tsurubuchi1996} ($1s_4$, $1s_2$) & Threshold--$10^3$ \\\cline{2-3}
    								 & Filipovic \textit{et al.}~\cite{Filipovic2000a} ($1s_2$) & 16--80 \\\cline{2-3}
    								 & Filipovic \textit{et al.}~\cite{Filipovic2000b} ($1s_5$--$1s_3$) & 20--80 \\\cline{2-3}
    								 & Khakoo \textit{et al.}~\cite{Khakoo2004} ($1s_5$--$1s_2$) & 14--100 \\
\hline
\end{tabular}
\caption{Summary of the curated electron-beam experiments and \textit{ab initio} calculation.}
\label{tab:crs-curation}
\end{table}
\begin{figure}
\input{figures/figure1.tex}
\caption{
Electron-impact argon cross section data from the curated electron-beam experiments and \textit{ab initio} calculation.
The reported standard-deviation error, if available from the reference, is indicated as an error bar.
}
\label{fig:crs-curation}
\end{figure}
The cross section data are curated from electron-beam experiments which at least notionally report their measurement accuracy~\cite{Gargioni2008,Pitchford2013}.
Table~\ref{tab:crs-curation} and Figure~\ref{fig:crs-curation} summarize the curated cross section data.
Almost all experimental data are limited to energy$>1eV$,
and very low-energy data is scarcely available.
The \textit{ab-initio} calculation (BSR) by Zatsarinny and Bartschat~\cite{Pitchford2013, Zatsarinny2013,BSR-data}
is also included in this study, which provides highly resolved data over a wide energy range.
Though its accuracy is not reported,
the data is considered credible based on its accurate prediction of atomic differential cross section from first-principles computation~\cite{Zatsarinny2013, Allan2006, Khakoo2011}.
%so we decided to include it in the inference with a conservatively assumed uncertainty.

%\subsubsection{A need for accounting the systematic error in the uncertainty}
\subsubsection{Discrepancies between datasets}

An observation from Figure~\ref{fig:crs-curation} is the large discrepancies among datasets.
Particularly for direct excitations in the $1-100eV$ range,
the datasets are scattered far outside the confidence intervals of each other,
indicating that their reported measurement errors cannot fully explain the discrepancy.
\par
This discrepancy is likely due to systematic errors that vary from experiment to experiment~\cite{Gargioni2008}.
There can be several factors contributing to such errors.
First, the detailed design of the electron gun varies between experiments as the energy range of interest usually spans from a few $eV$ to several thousands of $eV$~\cite{Gargioni2008}.
Also, the cross-beam technique, which is widely used for this type of experiment, is usually limited to relative measurements of the cross section,
so the measurement is scaled with a reference value.
The choice of this reference value can differ by experiments.
For the elastic collision, the widely-used relative flow techniques often use the cross section of helium~\cite{Srivastava1981, Gibson1996, Mielewska2004},
or the same cross section from other measurements~\cite{Panajotovic1997};
reflecting this point, Zatsarinny and Bartschat~\cite{Zatsarinny2004} also rescaled the experimental data from Buckman~\textit{et al.}~\cite{Buckman1983} to compare with BSR dataset.
Similarly for ionization, the measurement is sometimes normalized with respect to the cross section of hydrogen~\cite{Rapp1965};
or the absolute value is measured at only one energy, and the measurements at other energy points are respectively scaled~\cite{Straub1995}.
Likewise, the excitation cross sections are also normalized with previous measurements~\cite{Chutjian1981, Filipovic2000a, Filipovic2000b, Khakoo2004}.
Furthermore, many of these measurements are obtained by integrating the corresponding differential cross section over angle using a numerical quadrature,
where low-angle values are either extrapolated/adopted from other datasets~\cite{Srivastava1981, Panajotovic1997, Mielewska2004, Chutjian1981, Li1988, Filipovic2000a, Filipovic2000b, Khakoo2004}.
While Gibson~\textit{et al.}~\cite{Gibson1996} utilized a phase-shift analysis to infer from the differential cross section,
this involves a model-fitting procedure which likewise induces another systematic error.
The optical emission measurements also involve multiple excitation and cascade processes,
so measuring one of them requires approximation/estimation of the others~\cite{Schappe1994}.
\par
There is not sufficient prior knowledge available to separate and
indpendently quantify all these factors. However, simply neglecting
this discrepancy leads to a significantly misleading conclusion for
the uncertainty in the cross sections.  Instead, a probabilistic model
is introduced to account for the uncertainty implied by these
discrepancies.  The details of this model and its implications are
discussed further in Section~\ref{sec:bayes}.

\subsection{Swarm-analysis data}\label{subsec:swarm-data}

\subsubsection{Data chracterization}
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Databases & \makecell{Adopted (adjusted)\\ cross sections} & Reference\\
\hline
\multirow{3}{*}{Biagi/Biagi v7.1~\cite{Biagi1988, Biagi1989, Biagi-data}} & $\sigma_{el}$ ($<1eV$) & Haddad \& O'Malley~\cite{Haddad1982} \\
                                                                            & $\sigma_{ex}$ & BSR~\cite{BSR-data, Zatsarinny2013}\\
                                                                            & $\sigma_{ion}$ & Rapp \& Englander-Golden~\cite{Rapp1965}, \cite{Straub1995} \\
\hline
Hayashi~\cite{Hayashi2003, Hayashi-data} & \multicolumn{2}{|c|}{Compilation of 1960 literatures} \\
\hline
\multirow{3}{*}{IST-Lisbon~\cite{Alves2014, IST-Lisbon-data}} & $\sigma_{el}$ & Phelps~\cite{Yamabe1983} \\
                                           & $\sigma_{ex}$ & Hayashi~\cite{Hayashi2003}, \cite{Khakoo2004,Chilton1998,Weber2003,Drawin1967,Lee1973,Bretagne1986,Bretagne1982}\\
                                           & $\sigma_{ion}$ & Rapp \& Englander-Golden~\cite{Rapp1965}\\
\hline
\multirow{1}{*}{Morgan~\cite{Morgan-data}} & not specified. & Phelps and Hayashi$^*$~\cite{Pitchford2017}\\
\hline
\multirow{3}{*}{Puech~\cite{Puech1986, Puech-data}} & $\sigma_{el}$ ($0.014 \le \epsilon \le 4eV$) & Milloy \textit{et al.}~\cite{Milloy1977}\\
                                    & $\sigma_{el}$(otherwise) & Phelps~\cite{Frost1964}\\
                                    & $\sigma_{ex}$, $\sigma_{ion}$ & \cite{Bretagne1986}\\
\hline
\multirow{4}{*}{Phelps \cite{Frost1964,Tachibana1981, Phelps-data}} & $\sigma_{el}$ ($\epsilon<4eV$) & Milloy \textit{et al.}~\cite{Milloy1977}\\
                                                                                            & $\sigma_{el}$($\epsilon>8eV$) & \cite{Fletcher1972}\\
                                                                                            & $\sigma_{ex, total}$ & \cite{Schaper1969} \\
                                                                                            & $\sigma_{ion}$ & \cite{Smith1930} \\
%\hline
%\multirow{4}{*}{Milloy~\cite{Milloy1977}} & Estimated error: \\
%                                                                & $\le0.1eV$: $\pm6\%$ \\
%                                                                & $0.4-4.0eV$: $\pm8\%$ \\
%                                                                & $0.1-0.4eV$: $-20\sim+12\%$ \\
\hline
\multirow{4}{*}{Nakamura~\cite{Nakamura1988}} & $\sigma_{el}$ ($\epsilon\le2.5eV$) & Milloy \textit{et al.}~\cite{Milloy1977} \\
                                                                                & $\sigma_{el}$ ($\epsilon\ge15eV$) & \cite{Fon1983} \\
                                                                                & $\sigma_{ex, total}$ & \cite{Ferreira1983} \\
                                                                                & $\sigma_{ion}$ & Rapp \& Englander-Golden~\cite{Rapp1965} \\
\hline
\multirow{1}{*}{Haddad (1982) \cite{Haddad1982}}  & $\sigma_{el}$ ($\epsilon>1eV$) & Milloy \textit{et al.}~\cite{Milloy1977} \\
\hline
\end{tabular}
\caption{References of adopted cross sections in swarm-analysis datasets from LXCat community.
Authors of frequently adopted datasets are explicitly specified.}
\label{tab:lxcat-adoption}
\end{table}
Another type of widely used cross section data is based on swarm-analysis~\cite{Gargioni2008, Pitchford2013}.
The cross sections in these datasets are determined by requiring the transport properties and reaction rates as computed by using the cross sections in a zero-dimensional, two-term/multi-term Boltzmann solver to match those measured in the swarm parameter experiments.
Some widely used cross section datasets from swarm analysis are listed in Table~\ref{tab:lxcat-adoption}, and
Table~\ref{tab:swarm-parameter} summarizes the swarm parameter measurements used in this work.  Further, these data
are shown in Figure~\ref{fig:swarm-parameter} and Figure~\ref{fig:swarm-parameter-ex}.

%These swarm parameter experiments measure more direct observables,
%so the scattering among the experiments is not significant compared to the electron-beam experiments,
%thus being subject to less uncertainty.
%The swarm-analysis can also provide the cross sections at low energy range below $1 eV$,
%which are not available from the electron-beam experiments.

\par
\begin{table}[tbp]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Type & Reference & Swarm parameters & Condition \\
\hline
\multirow{9}{*}{Transport} & Townsend \& Bailey~\cite{Townsend1922, Pitchford2013} & $D_T / \mu$ & \\\cline{2-4}
                                            & Pack \& Phelps~\cite{Pack1961} & $W = \mu E$ & $77K$, $300K$ \\\cline{2-4}
                                            & Warren \& Parker~\cite{Warren1962} & $D_T / \mu$ & $77K$, $88K$ \\\cline{2-4}
                                            & Robertson \& Rees~\cite{Robertson1972} & $D_L / \mu$ & $90K$, $700Torr$/$800Torr$ \\\cline{2-4}
                                            & Robertson~\cite{Robertson1977} & $W$ & $89.6K$, $293K$ \\\cline{2-4}
                                            & Milloy \& Crompton~\cite{Milloy1977ratio} & $D_T/\mu$ & $294K$ \\\cline{2-4}
                                            & Kucukarpaci \& Lucas~\cite{Kucukarpaci1981} & $W$, $D_L\mu$ & $300K$ \\\cline{2-4}
                                            & Al-Amin \& Lucas~\cite{AlAmin1987} & $D_T/\mu$ & \\\cline{2-4}
                                            & Nakamura \& Kurachi~\cite{Nakamura1988} & $W$, $D_L/N$ & $300K$ \\
\hline
\multirow{3}{*}{Ionization} & Golden \& Fisher~\cite{Golden1961} & \multirow{3}{*}{$\alpha_{ion}$} & \\\cline{2-2}\cline{4-4}
                                        & Kruithof~\cite{Kruithof1940} &  & $273.15K$ \\\cline{2-2}\cline{4-4}
                                        & Specht \textit{et al.}~\cite{Specht1980} &  & $300K$ \\
\hline
\multirow{6}{*}{Excitation} & Tachibana~\cite{Tachibana1986} & \multirow{6}{*}{$\alpha_{ex}$ ($1s_5$--$1s_2$)} & \\\cline{2-2}\cline{4-4}
                                         & Biagi~\cite{Biagi1988, Biagi1989, Biagi-data} & & \multirow{5}{*}{$300K$} \\\cline{2-2}
                                         & BSR~\cite{Pitchford2013, Zatsarinny2013,BSR-data} & & \\\cline{2-2}
                                         & Hayashi~\cite{Hayashi2003, Hayashi-data} & &  \\\cline{2-2}
                                         & IST-Lisbon~\cite{Alves2014, IST-Lisbon-data} & &  \\\cline{2-2}
                                         & Puech~\cite{Puech1986, Puech-data} & & \\\cline{2-2}
\hline
\end{tabular}
\caption{Summary of swarm parameter experiment data.}
\label{tab:swarm-parameter}
\end{table}
\begin{figure}
\input{figures/figure3.tex}
\caption{
Swarm parameter experiment data used for validation of the calibrated cross sections:
(a) drift velocity,
(b) the ratio of longitudinal diffusivity to mobility,
(c) the ratio of transverse diffusivity to mobility, and
(d) the reduced ionization coefficient.
The error bar, if available, indicates the reported standard deviation of the measurement. 
}
\label{fig:swarm-parameter}
\end{figure}
\begin{figure}
\input{figures/figure3-1.tex}
\caption{
Swarm parameter data used for validation of the calibrated cross sections:
the reduced excitation coefficient to the level (a) $1s_5$, (b) $1s_4$, (c) $1s_3$, and (d) $1s_2$.
The error bar, if available, indicates the reported standard deviation of the measurement. 
}
\label{fig:swarm-parameter-ex}
\end{figure}
The figures show that, the scatter among datasets for the same conditions is small compared to that of the electron-beam experiments.
While the ionization Townsend coefficient from Specht \textit{et al.}~\cite{Specht1980} deviates from other experiments at low energy,
the authors recognized that in this regime their measurements include contributions from photoelectric emission by the metastables.
\par
The experimental data for the direct excitation rate coefficients is scarce,
since it is difficult to isolate these collision processes from others, especially radiative de-excitations.
While we use the experimental data from Tachibana~\cite{Tachibana1986} who estimated these radiative de-excitation rates from the emission spectroscopy,
we also adopt the swarm-analysis data from the LXCat community~\cite{Pitchford2013, Biagi-data, BSR-data, Hayashi-data, IST-Lisbon-data, Puech-data},
as shown in Figure~\ref{fig:swarm-parameter-ex}.
The excitation rate coefficients are obtained using a zero-dimensional Boltzmann solver (\texttt{BOLSIG+}~\cite{Hagelaar2005}),
with the nominal cross section datasets~\cite{Biagi-data, BSR-data, Hayashi-data, IST-Lisbon-data, Puech-data}.
The direct excitation rates to $2p$-levels are also computed from the same datasets,
which are then assumed to be radiatively de-excited to $1s$-levels based on radiative transition probabilities~\cite{Wiese1969}.
This approximation has been used for comparison with the experiment~\cite{Puech1986, Alves2005, Pitchford2013}.

\subsubsection{Implicit, inter-dependent swarm-analysis datasets}

The cross section datasets from swarm analysis are, however,
not readily usable for quantifying uncertainty in the cross sections.
First of all, the cross sections are calibrated in a least-square sense,
and the uncertainties in the experiments are not backward-propagated toward the cross sections.
Thus, most sources only provide the maximum-likelihood estimate of the cross section
and do not attempt to assess its uncertainty.
To our knowledge,
the only swarm-analysis dataset which does provide its uncertainty
is the elastic momentum-transfer cross section at low energy by Milloy \textit{et al.}~\cite{Milloy1977},
where the uncertainty is estimated via a sensitivity analysis.
\par
%\todo[inline]{If this paragraph below $\downarrow$ is striking too much, we may shorten/omit it.}
\begin{figure}
\input{figures/figure2.tex}
\caption{
Elastic momentum-transfer cross sections from swarm-analysis datasets:
(a) on the overall energy range, and
(b) on $\epsilon\in[0.014, 4]$ ($eV$),
to show the agreement with the data from Milloy \textit{et al.}~\cite{Milloy1977}.
}
\label{fig:lxcat-elastic}
\end{figure}
A more fundamental challenge in using these datasets lies in their inter-dependency.
The swarm parameters depend on the electron energy distribution function, which is determined by the entire set of collision processes.
%Since it can be computationally prohibitive to calibrate all the collision processes together,
The set of collision processes that can be inferred from the transport/chemistry data is not unique,
unless the experimental condition reduces the number of possible collision processes~\cite{Crompton1994, Gargioni2008}.
This is possible only for the elastic momentum-transfer processes in the low-energy range for noble gases~\cite{Crompton1994, Gargioni2008, Milloy1977}.
A common practice for other collision processes is to calibrate only a target collision process, while the other necessary cross sections are taken from the literature, sometimes with mild adjustments.
As a result, the cross sections from swarm analysis datasets often show small discrepancies among each other,
though this result does not necessarily imply that the actual uncertainty is small.
The elastic momentum-transfer cross section shown in Figure~\ref{fig:lxcat-elastic} is one stark example.
%\todo{SWC: Have a feeling that this example may be somewhat unfair? If so, we can omit this Figure~\ref{fig:lxcat-elastic} example.}
While these datasets are mildly scattered either for $\epsilon < 0.014 eV$ or for $\epsilon > 4 eV$,
all of them are strikingly well aligned within $\epsilon\in[0.014, 4]$ interval, except a small variation at the Ramsauer minimum.
While it may be tempting to say that the cross section in this range has an extremely low uncertainty,
it is rather the result of everyone adopting and mildly adjusting the dataset from Milloy \textit{et al}~\cite{Milloy1977}.
Table~\ref{tab:lxcat-adoption} shows these swarm-analysis datasets which are known to have adopted Milloy \textit{et al.}~\cite{Milloy1977} with mild adjustments.
%While the cross section values in this range has been considered accurate,
Employing all these datasets independently will induce a strong, artificial bias to that from Milloy~\textit{et al}~\cite{Milloy1977}.
While the elastic collision may be considered accurate on this range,
almost all other cross sections---which are not deemed accurate as the momentum-transfer---are also adopted from the literatures as shown in Table~\ref{tab:lxcat-adoption},
thus having an inter-dependency with each other.
%\par
%Of course, this does not mean that the data in this range is entirely not credible.
%Rather, there are reasons to believe that the cross section value in this range can be deemed accurate:
%in this low-energy range, the elastic collision is the only dominant process and thus no other collision cross sections need to be adopted or calibrated;
%and the swarm-parameter experiment data used for calibration is not subject to either a large measurement error or discrepancy against other experiments.
%However, from a statistical viewpoint, this significantly hinders evaluating the uncertainty without bias,
%as the datasets are not independent and rather have a strong, artificial correlation with each other.
%For example, BSR dataset from \textit{ab initio} calculation, also shows a small difference from other datasets in Figure~\ref{fig:lxcat-elastic}~(b),
%though not perfectly aligned with them.
%Calibrating the cross section with all datasets equally weighted will lead to a result heavily biased to that from Milloy~\textit{et al}~\cite{Milloy1977}.
%While this may cause only a small difference for the momentum-transfer process,
%almost all other cross sections---which are not deemed accurate as the momentum-transfer---are also adopted from the literatures, thus having an inter-dependency with each other.
%Table~\ref{tab:lxcat-adoption} summarizes the collision cross sections in these swarm-analysis datasets that are adopted or mildly adjusted from other literatures.
\par
For these reasons, the cross sections from swarm-analysis are not used for calibration in this work.

\subsubsection{Swarm-parameter experiments as a validation case}
In principle,
the swarm parameter experiment data in Table~\ref{tab:swarm-parameter}
can be also used for Bayesian inference.
This requires an inverse problem of finding the semi-empirical cross section models,
whose outputs through the Boltzmann equation match the swarm parameter measurements.
This is in essence a more comprehensive swarm-analysis:
the entire set of cross sections would be calibrated together;
and the associated uncertainty would be evaluated,
which involves much larger statistical sampling than simply fitting the models, even with a simplified Boltzmann model such as \texttt{BOLSIG+}~\cite{Hagelaar2005}.
\par
In order to avoid this increase in the sampling cost,
it is decided to use only the direct cross section measurements in Table~\ref{fig:crs-curation}
for the Bayesian inference procedure.
The swarm parameter experiment data in Table~\ref{tab:swarm-parameter}
are instead used for validation of the calibrated models resulting from the Bayesian inference, as shown in Section~\ref{sec:result}.

%\begin{tabular}{|c|c|c|c|}
%\hline
%Databases & Cross section ref. & Experiments ref.\\
%\hline
%\multirow{3}{*}{Biagi/Biagi v7.1} & $<1eV$: \cite{Haddad1982} (adjusted) & Drift vel: \cite{Nakamura1988} ($<0.25\%$ at low $E/N$, $<1\%$ at high $E/N$)\\
%& & Diff. co: \cite{Milloy1977,Milloy1977ratio,Saelee1976,Kucukarpaci1981,Levine1964} ($<0.25\%$ at low $E$, $<3\%$ at $E\le200kV/cm$)\\
%& & experiment from BSR group~\cite{Allan2006}, \cite{Oliveira2011,Sahin2010} (not specified)\\
%\hline
%Hayashi & \multicolumn{2}{|c|}{Compilation of 1960 literatures~\cite{Hayashi2003} (error not provided)} \\
%\hline
%\multirow{3}{*}{IST-Lisbon} & mmt. trsf: Phelps~\cite{Yamabe1983} & $2-25\%$ error (including inelastic exp., \cite{Alves2014})\\
%& excitation: Hayashi~\cite{Hayashi2003}, \cite{Khakoo2003,Chilton1998,Weber2003,Drawin1967,Lee1973,Bretagne1986,Bretagne1982}
%& Drift velocity: \cite{Nielsen1936,Bowe1960,Pack1961,Wagner1967,Robertson1977,Christophorou1979,Kucukarpaci1981,Nakamura1988} (Figure~\ref{fig:yanguas2005fig7-8}, left)\\
%& ionization: \cite{Rapp1965} & Chracteristic energy: \cite{Townsend1922,Townsend1923,Warren1962} (Figure~\ref{fig:yanguas2005fig7-8}, right) \\
%\hline
%\multirow{2}{*}{Morgan} & not specified. & not specified. \\
%& {\tiny \enquote{some overlap with datasets in Phelps and Hayashi} }\cite{Pitchford2017} & \\
%\hline
%\multirow{3}{*}{Puech} & M. T. $0.014-4eV$: Milloy\cite{Milloy1977} & drift vel: \cite{Robertson1977,Kucukarpaci1981} (Fig~\ref{fig:puech1986-fig6}) \\
%& M. T. othewise: outdated Phelps\cite{Frost1964} & Ch. energy: \cite{Dutton1975,Milloy1977ratio,Lakshminarasimha1977} ($<10\%$) \\
%& Inelastic: \cite{Bretagne1986} & \\
%\hline
%\multirow{4}{*}{Phelps (\cite{Frost1964,Tachibana1981})} & mmt. trsf for $<4eV$: Milloy~\cite{Milloy1977}
% & Drift velocity (\cite{Frost1964}, outdated): \cite{Warren1962,Townsend1922,Pack1961,Bowe1960,Nielsen1936,Haddad1982} (Figure~\ref{fig:frost1964-fig3}) \\
% & mmt. trsf for $>8eV$: \cite{Fletcher1972}& $O_2-Ar$ mixture exp.: \cite{Tachibana1981} ($<10\%$)\\
% & total excitation: \cite{Schaper1969} & \\
% & ionization: \cite{Smith1930} & \\
%\hline
%\multirow{4}{*}{Milloy~\cite{Milloy1977}} & Estimated error: & Drift vel: \cite{Robertson1977} ($90K$: rms $1\%$, $293K$: rms $0.5\%$, max $1\%$) \\
%& $\le0.1eV$: $\pm6\%$ & diff. coeff. \cite{Milloy1977ratio} ($294K$: rms $1.5\%$, max $3\%$) \\
%& $0.4-4.0eV$: $\pm8\%$ & \\
%& $0.1-0.4eV$: $-20\sim+12\%$ & \\
%\hline
%\multirow{4}{*}{Nakamura~\cite{Nakamura1988}} & M.T. $\le2.5eV$: \cite{Milloy1977} & Double shutter drift \cite[Figure 5]{Nakamura1988}\\
%& M.T. $\ge15eV$: \cite{Fon1983} & Drift vel.: $<2\%$, rms $\lesssim1\%$ \\
%& Excitation: \cite{Ferreira1983} & Long. diff. coeff.: $<10\%$, rms not specified \\
%& Ionization: \cite{Rapp1965} & \\
%\hline
%\multirow{2}{*}{Haddad (1982) \cite{Haddad1982}} & Little extension of Milloy~\cite{Milloy1977} & \cite{Robertson1977,Milloy1977ratio} (error: \cite[Fig 3]{Haddad1982}\\
%& M.T. $>1eV$: Milloy~\cite{Milloy1977} & \\
%\hline
%\end{tabular}


==> sections-orig/intro.tex <==
\section{Introduction}

%\todo[inline]{more citations in the paragraph below $\downarrow$? RDM:
%seems OK, but this paragraph needs to be fleshed out with more physics
%context, particularly role in boltzmann equation and in determining
%reaction and transport characteristics, also need a brief review of
%representations of cross sections for use in plasma simulations}
Determining cross sections for atomic and molecular collision processes is crucial to the accuracy of plasma discharge model predictions~\cite{Gargioni2008}.
Most macroscopic observables of plasma, such as pressure or temperature,
are features of the energy distribution functions of the particles that comprise the plasma~\cite{Ferziger1973}.
The evolution of these energy distribution functions is governed by the species Boltzmann equation, in which the cross sections appear in the collision term that represents the effects of particle interactions.
%The microscopic, molecular collisions are the major driving force of the evolution of these distributions,
%which is described by Boltzmann equation.
Chemical reactions and transport processes are the macroscopic averages of these collision processes~\cite{Vlcek1989, Bultel2002, Kapper2011}, and
thus are determined by both the cross sections themselves and the energy distributions.
In this context, electron-impact collisions are particularly important for modeling non-equilibrium plasmas~\cite{Pitchford2013, Pitchford2017}, where the energy distribution functions cannot be determined from equilibrium considerations.
%As themselves, they determine the fundamental plasma chemistry and transport processes. 
%They further determines the form of electron energy distribution function (EEDF)~\cite{Pitchford2013, Pitchford2017},
%which in turn impacts plasma chemistry and transport.
\par
%\todo[inline]{Add citations for this paragraph $\downarrow$.}
Because of these dependencies, particle collision cross sections are necessary for a plasma discharge model.
They are clearly essential for simulations based on the Boltzmann equations, where they appear explicitly.
In particle-based Monte-Carlo simulations of the Boltzmann equation,
these cross sections are used to statistically determine the collision rates~\cite{Oran1998, Bird1994, Birdsall1991, Vahedi1993, Birdsall2004}.
In grid-based Boltzmann equation simulations, on the other hand,
the collision rates are evaluated deterministically as expectations over the evolving distributions.
In either case, the cross sections---represented as functions of electron energy,
either by an analytical model or a tabulated data---are direct inputs to the model.
Further, even in fluid-based models where the cross sections do not
appear explicitly in the model PDEs, the input data---specifically,
reaction rates and transport properties---are dependent on the
underlying cross sections~\cite{Hagelaar2005}.
Because of this importance, the characterization of collision
cross sections has been a focus of experimental measurements for many
decades and, more recently, \textit{ab initio} quantum mechanics
simulations.  This work has resulted in numerous databases of
cross sections, e.g.,~
\par
%\todo[inline]{The paragraph below $\downarrow$ is written
%  assuming that the importance of collision cross section is
%  established in the paragraph above $\uparrow$.}
%
%\todo[inline]{RDM: Need UQ references in the following\\SWC: some citations are added}

Unfortunately, the determination of collision cross sections is
subject to uncertainties. These uncertainties arise from experimental
or numerical errors in measuring the cross sections, and from
uncharacterized systematic errors intrinsic to these studies.
% \cite{Gargioni2008}.
Because of the importance of the cross sections
to the characteristics of a plasma, their uncertainty results in
uncertainties in the predicted plasma properties when the
cross sections are used in a plasma simulation. To quantify
uncertainties in the predictions, it is necessary to quantify the
uncertainties in the cross sections. Such uncertainty quantification
(UQ) allows the reliability of simulation predictions to be assessed
and provides a basis for interpreting discrepancies between
simulations and experiments.
% ~\cite{Stuart2010, Smith2013}.
A representation of collision
cross sections for use in a plasma simulation should therefore include
uncertainties. Here we propose an uncertain cross section formulation
which is informed by data from multiple sources using Bayesian
inference.
% ~\cite{Kennedy2001, Rasmussen2006, Foreman-Mackey2013}.
To illustrate the cross section uncertainty quantification process,
we consider six important electron collision processes with the ground-state argon atom.
The collision processes are elastic momentum-transfer,
direct ionization, and direct excitation to the four $1s$ excited
states. The same UQ process can be similarly applied to any other
collision process, assuming the necessary data are available.

%RDM Above includes a streamlined version of the following, please check
%that it captures the important points.
%
%% Accurate identification of a cross section does not mean presenting the absolutely true value,
%% which in fact we deem not accessible ever.
%% Nor does it mean simply presenting the best-fitting value that produces the best prediction for most plasma simulations.
%% There is always the lack of our knowledge about a cross section,
%% and such ignorance must be reduced for the accurate identification of the cross section.
%% Such reduction, of course, is predicated upon the evaluation of the ignorance in a quantitative way.
%% Uncertainty quantification (UQ), particularly the Bayesian inference, can provide a systematic framework for this.
%% Based on our prior knowledge and observations from the experiments,
%% the lack of our knowledge can be quantitatively evaluated as uncertainty in a probabilistic description.
%% Such uncertainty can also be utilized to analyze the impacts on higher-level predictions
%% where the cross sections are used as model inputs.
%% Our goal is to develop a Bayesian inference process where the uncertainty of a cross section
%% can be evaluated from various measurement datasets.
%% While there are a massive number of species and collisions,
%% we mainly use the datasets for 6 major electron-argon collision processes
%% to present our UQ process: elastic momentum-transfer, direct ionization, and direct excitation to 4 $1s$-levels.
%% The same framework can be similarly applied to any other collision processes.
%\par \todo[inline]{Paragraph $\downarrow$: how much details do we
%  need?}

There have been many studies to measure electron-impact cross sections
in argon. They are generally of three types: electron beam
experiments, swarm experiments and \emph{ab initio} quantum
calculations. These experiments and their uncertainties are discussed briefly
below. Detailed reviews of cross section measurements are available
in.
% ~\cite{Bederson1971, Gargioni2008, Pitchford2013, Pitchford2017}.


Electron-beam experiments measure the scattering of a mono-energetic
electron beam, to determine differential cross sections at specific
energies and angles.
%  \cite{Bederson1971, Gargioni2008}.
Combined with optical techniques, they
can also measure excitation cross sections.
%  \cite{Filippelli1994, Tachibana1986, Chilton1998}.
These are direct
measurements of the cross sections, which are generally reported with
an assessment of the experimental uncertainties. However, the
measurements also involve systematic errors that are difficult to
assess and vary from experiment to experiment.
% ~\cite{Gargioni2008}.
As
a result there are discrepancies among datasets from electron-beam
experiments that are large compared to their reported uncertainties.

Electron swarm experiments measure electron transport parameters in
swarms of electrons, which depend on the collision cross sections.
% \cite{Bederson1971, Gargioni2008, Pitchford2013}.
Obtaining the cross sections from the transport properties determined in the swarm experiments
requires an inference procedure involving the (usually simplified)
Boltzmann equation, in which many collision processes are active
simultaneously.
% ~\cite{Milloy1977, Haddad1982, Nakamura1987, Biagi1989, Alves2005}.
In this analysis, it is often necessary to employ
prior information on cross sections from other sources, either for a
certain energy range or for a particular collision process.
% \cite{Pitchford2013}.
Uncertainties in the inferred cross sections
arise from the error in measuring the electron transport properties,
errors arising from the simplifications in the analysis and from the
uncertainties in the cross sections from other sources that are adopted
in the analysis. The latter two uncertainties generally go
uncharacterized.

%\todo[inline]{RDM: need a few sentences about BSR data, the nature of
%  the computations, and its reliability/uncertainty\\ SWC: added some sentences.}
Aside from experiments,
\emph{ab initio} quantum calculations also provide cross section data.
% ~\cite{Pitchford2013, Pitchford2017}.
These calculations involve the wavefunctions of a colliding electron and atom solved
through approximate forms of Schr\"{o}dinger's equation.
The cross section is computed as a dependent variable.
% ~\cite{Zatsarinny2013, Mceachran2014, Gangwar2012, Djuissi2022}.
Among various \emph{ab initio} datasets, the BSR data provides a comprehensive set of
electron-argon collision cross sections.
% ~\cite{Zatsarinny2004, Zatsarinny2013, Zatsarinny2014, Allan2006, Khakoo2011}.
The resulting cross section data for noble gases agree well with experimental data.
%considering that it is computed from the first principle without employing other empirical data.
While the errors arising from the approximate model remain uncharacterized,
the data is considered credible based on its accurate prediction and its low dependency on other (uncertain) sources.


Most reviews of cross section datasets from different sources
% ~\cite{Gargioni2008, Pitchford2013, Pitchford2017}
compare them
and report their discrepancies. These discrepancies can be interpreted
as arising from the unquantified uncertainties associated with the
various datasets as described above. However, naively taking these
discrepancies as a direct measure of uncertainty would be problematic
for two reasons. First, such a characterization would not represent
the correlation of errors at different collision energies. Second, in
swarm analysis the datasets are often inter-dependent because they
share sources of externally provided cross section
data
% ~\cite{Pitchford2013}.
As a result, the discrepancy among swarm
datasets understates the uncertainties.

%\par
%One reason is because cross sections are often not directly measurable, even with electron-beam experiments.
%As a result, most experiments involve some inference procedures with assumptions.\todo{Elaborate more with examples.}
%Uncertainties underlying in this procedure are usually hard to be quantified,
%and the reported accuracies of the experiments are often notional.
%\par
%Another reason is the difficulty of identifying correlation along electron energy space.
%While a cross section must be a function of energy and thus cross section values at any energy points are dependent on each other,
%its true functional form is not known (and probably will never be).
%So it is necessary to 
\par In this paper, we develop an uncertain representation of
electron-argon neutral collision cross sections as a function of collision
energy. The approach accounts for both the estimated uncertainty in the
available data and the systematic errors exposed by the inconsistency
between datasets. The representation is based on semi-empirical
cross section models which include a few tunable
parameters,
% ~\cite{Gargioni2008,Haddad1982,Bretagne1986,Kim1994},
with
an expectation that these parametric representations will be sufficient
to capture the features of the cross sections that are essential to reaction rates and transport parameters in collisional plasma simulations.  For other applications where one is interested in the cross section at specific energies, rather than integrated quantities, a richer representation may be necessary.
%
The
model parameters are considered uncertain, but to account for any errors
introduced by the semi-empirical model form and the discrepancies
introduced by unquantified systematic errors as discussed above, a
Gaussian process representation of the error is also included.
% ~\cite{Kennedy2001}.
A Gaussian process model is non-parametric, probabilistic
representation of a function that is characterized by a number of hyperparameters.  In the present work, Gaussian processes provide a flexible way to account for errors about which we do not have sufficient information to pose a parametric model.

For each collision, the semi-empirical model parameters and the
Gaussian process hyperparameters are determined, with uncertainties,
using Bayesian inference from the experimental and \emph{ab initio}
computational data described above.
Because the aforementioned errors in the cross sections derived from swarm experiments
are confounding and difficult to characterize,
these results are not used for the Bayesian inference.
Instead, the swarm data are reserved for
validation of the probabilistic cross section model. Details of the
data used for model calibration and validation are provided in
Section~\ref{sec:curation}.

In the remainder of the paper, the data are described in some detail
(Section~\ref{sec:curation}) and then the semi-empirical cross section
models are introduced (Section~\ref{sec:model}). The Bayesian
calibration formulation is described in Section~\ref{sec:bayes}, and
the results of the Bayesian calibration and validation for three
different formulations of the probabilistic error model are presented
in Section~\ref{sec:result}. Finally, concluding remarks are provided
in Section~\ref{sec:conclusion}.


%The goal of this paper is to properly assess the cross section uncertainties that are essential for the plasma reaction and transport processes.
%It is crucial to have a formulation that can quantitatively reflects our knowledge under statistical principles,
%and still can be evaluated in a computationally efficient manner.
%We employ a Bayesian approach to infer cross section uncertainties from measurement data.
%Since the swarm parameters are indirectly determined by the cross sections and dependent on
%additional modeling choices, it was decided to infer the cross
%sections using only the direct measurements and reserve the swarm-analysis data for validation of the resulting model.
%The detailed decision process for this will be presented in Section~\ref{sec:curation}.
%\par
%The cross sections $\sigma(\epsilon)$ were characterized using
%semi-empirical models $f(\epsilon;\vec{A})$, where $\epsilon$ denotes
%energy and $\vec{A}$ represents the model
%parameters~\cite{Gargioni2008,Haddad1982,Bretagne1986,Kim1994}.  The
%motivation for this choice was the expectation that these models,
%coupled with their parametric uncertainty, would be sufficient to
%capture the essential features of the cross sections that are relevant
%to the plasma reaction and transport processes.

%This is particularly true for
%
%
%The goal of this paper is to assess the uncertainties of the electron-impact collision cross sections that are crucial for
%under statistical principles.
%Since the swarm parameters are
%indirectly determined by the cross sections and dependent on
%additional modeling choices, it was decided to infer the cross
%sections using only the direct measurements and reserve the swarm
%parameter data for validation of the resulting model.
%
%
%Our strategy to utilize these data will be presented based on their characteristics.
%In essence, we infer 
%
%We limit our demonstration to 6 main electron-impact processes of argon plasma (elastic momentum-transfer, direct ionization and 4 $1s$-level direct excitations);
%however, application to other collision processes must be straightforward.


==> sections-orig/intro_old.tex <==
\section{Introduction}

\todo[inline]{more citations in the paragraph below $\downarrow$?}
Identifying cross-sections of molecular collision processes is crucial for accurate prediction of plasma physics~\cite{Gargioni2008}.
Reaction rates of plasma chemistry and plasma transport properties are determined by these collision processes~\cite{Vlcek1989, Bultel2002, Kapper2011}.
Amongst all, electron-impact collisions are particularly important for non-equilibrium plasma~\cite{Pitchford2017}.
Electron-impact collisions determines the specific form of electron energy distribution function (EEDF)~\cite{Pitchford2013, Pitchford2017},
which further impacts plasma chemistry and transport.
%\todo[inline]{Limit the scope to argon plasma somewhere.}
\par
\todo[inline]{The paragraph below $\downarrow$ is written assuming that the importance of collision cross-section is established in the paragraph above $\uparrow$.}
Accurate identification of a cross-section does not mean presenting the absolutely true value,
which in fact we deem not accessible ever.
Nor does it mean simply presenting the best-fitting value that produces the best prediction for most plasma simulations.
There is always the lack of our knowledge about a cross-section,
and such ignorance must be reduced for the accurate identification of the cross-section.
Such reduction, of course, is predicated upon the evaluation of the ignorance in a quantitative way.
Uncertainty quantification (UQ), particularly the Bayesian inference, can provide a systematic framework for this.
Based on our prior knowledge and observations from the experiments,
the lack of our knowledge can be quantitatively evaluated as uncertainty in a probabilistic description.
Such uncertainty can also be utilized to analyze the impacts on higher-level predictions
where the cross-sections are used as model inputs.
Our goal is to develop a Bayesian inference process where the uncertainty of a cross-section
can be evaluated from various measurement datasets.
While there are a massive number of species and collisions,
we mainly use the datasets for 6 major electron-argon collision processes
to present our UQ process: elastic momentum-transfer, direct ionization, and direct excitation to 4 $1s$-levels.
The same framework can be similarly applied to any other collision processes.
\par
\todo[inline]{Paragraph $\downarrow$: how much details do we need?}
There have been significant efforts to identify the electron-impact cross sections of argon plasma.
These efforts are characterized in mainly two categories:
direct cross-section measurements and swarm-parameter analysis.
%These efforts are characterized in mainly two approaches:\todo{elaborate them more.}
%electron-beam experiments and swarm-parameter analysis.
In the first category,
the cross-sections are directly measured either by electron-beam experiments or by \textit{ab initio} calculations.
Electron-beam experiments measure the scattering of a mono-energetic electron beam,
providing differential cross sections at specific energies and angles.
Combined with optical techniques, they can also provide excitation cross sections.
Recent developments in numerical techniques for quantum physics also enabled direct calculation of the cross-sections based on first principle.
On the other hand, swarm-analysis infers cross sections from measurements of transport properties,
which are relatively easier to measure with more accuracy.
While electron energy distribution function (EEDF) should be inferred with several approximations and simplifications,
the swarm-analysis can provide absolute cross-sections for impact energies below $1 eV$.
Detailed reviews of cross section measurements are available~\cite{Gargioni2008, Pitchford2013, Pitchford2017}.
In Section~\ref{sec:curation}, we curate and categorize the measurement data for these cross sections into direct measurements and swarm-analysis.
\par
Thanks to such efforts, generic forms and values of electron-impact cross sections are well-known.
Their underlying uncertainties, however, have not been assessed well.
While electron-beam experiments provide direct cross-section measurements with explicitly reported accuracy,
these measurements involve systematic errors varying from experiments to experiments~\cite{Gargioni2008}.
Most of these biases are difficult to assess,
and as a result there are a large discrepancies among the datasets from electron-beam experiments, compared to their reported accuracies.
On the other hand,
despite accurate measurement of the transport properties,
the swarm-analysis relies upon the inference procedure with a simplified Boltzmann equation,
where a set of many collision processes interact with each other in an implicit and nonlinear way.
As a result, the dependence of the swarm parameters on the cross-sections cannot be expressed with a simple, explicit algebraic relation,
and likewise the uncertainty of the inferred cross-section remains implicit.
The correlation between the inferred cross-sections is also not well investigated for the same reason.
\par
Most reviews of cross-section datasets~\cite{Gargioni2008, Pitchford2013, Pitchford2017}
merely compare them and report their discrepancies.
Naively taking these discrepancies as uncertainties can be problematic,
since it would only represent a marginal probability at a single electron energy, entirely missing the correlation along the electron energy space.
Furthermore, these discrepancies can be misleading when the datasets are inter-dependent.
This is indeed the case for swarm-analysis datasets~\cite{Pitchford2013},
where it is often necessary to adopt cross sections from other sources, either for a certain energy range or for a collision process.
As a result, a small discrepancy among datasets is often due to sharing the same source, not necessarily representing a small uncertainty.
%\par
%One reason is because cross sections are often not directly measurable, even with electron-beam experiments.
%As a result, most experiments involve some inference procedures with assumptions.\todo{Elaborate more with examples.}
%Uncertainties underlying in this procedure are usually hard to be quantified,
%and the reported accuracies of the experiments are often notional.
%\par
%Another reason is the difficulty of identifying correlation along electron energy space.
%While a cross section must be a function of energy and thus cross section values at any energy points are dependent on each other,
%its true functional form is not known (and probably will never be).
%So it is necessary to 
\par
In this paper, we assess the cross-section uncertainties of the electron-argon collision processes under Bayesian framework.
Due to the implicit dependence of the swarm-parameter measurements on cross-sections,
it was decided to infer the cross-sections using only the electron-beam measurements
and reserve the swarm-analysis data for validation of the resulting model.
Details of this decision process will be discussed in Section~\ref{sec:curation}.
%The cross-sections $\sigma(\epsilon)$ were characterized using
Semi-empirical models with a few parameters are used to characterize the cross-sections~\cite{Gargioni2008,Haddad1982,Bretagne1986,Kim1994},
with an expectation that their parametric uncertainty would be sufficient to
capture the essential features of the cross-sections that are relevant to the plasma reaction and transport processes.
\par
Formulating a proper likelihood model is crucial to accurately assess the uncertainty underlying the data.
The parametric uncertainty, of course, is not the only source of the cross-section uncertainty.
Part of the error between the model and the data can be attributed to the inherent inadequacy of the cross-section model.
Furthermore, as described earlier, systematic errors of the experiments can also induce the discrepancies, even among the datasets.
This is particularly true for the electron-beam data,
where the discrepancy is significant and cannot be explained by their reported observation errors.
A naive likelihood that does not reflect these factors can lead us to a misleading conclusion about the underlying uncertainty of the cross-sections.
Here, the combined effects of this systematic error and any inherent inadequacy in the semi-empirical
cross section model is represented statistically using a Gaussian process~\cite{Kennedy2001}.
\par
In Section~\ref{sec:curation},
we summarize the curated data for the 6 collision processes, both for the direct measurement and the swarm-analysis.
In Section~\ref{sec:model},
the semi-empirical cross-section models chosen for the Bayesian inference are introduced.
In Section~\ref{sec:bayes},
the framework for the Bayesian inference is introduced,
and the likelihood and the posterior probability are formulated.
In Section~\ref{sec:result},
the inferred parametric uncertainty of the cross-sections are reported.
This is compared with the result of the naive likelihood,
demonstrating the importance of the systematic error modeling in the Bayesian framework.
The inferred uncertainties are then propagated using a 0-D Boltzmann solver,
and validated with the swarm-parameter data.
In Section~\ref{sec:conclusion},
we summarize our study and future works.

%The goal of this paper is to properly assess the cross-section uncertainties that are essential for the plasma reaction and transport processes.
%It is crucial to have a formulation that can quantitatively reflects our knowledge under statistical principles,
%and still can be evaluated in a computationally efficient manner.
%We employ a Bayesian approach to infer cross-section uncertainties from measurement data.
%Since the swarm parameters are indirectly determined by the cross sections and dependent on
%additional modeling choices, it was decided to infer the cross
%sections using only the direct measurements and reserve the swarm-analysis data for validation of the resulting model.
%The detailed decision process for this will be presented in Section~\ref{sec:curation}.
%\par
%The cross sections $\sigma(\epsilon)$ were characterized using
%semi-empirical models $f(\epsilon;\vec{A})$, where $\epsilon$ denotes
%energy and $\vec{A}$ represents the model
%parameters~\cite{Gargioni2008,Haddad1982,Bretagne1986,Kim1994}.  The
%motivation for this choice was the expectation that these models,
%coupled with their parametric uncertainty, would be sufficient to
%capture the essential features of the cross-sections that are relevant
%to the plasma reaction and transport processes.

%This is particularly true for
%
%
%The goal of this paper is to assess the uncertainties of the electron-impact collision cross sections that are crucial for
%under statistical principles.
%Since the swarm parameters are
%indirectly determined by the cross sections and dependent on
%additional modeling choices, it was decided to infer the cross
%sections using only the direct measurements and reserve the swarm
%parameter data for validation of the resulting model.
%
%
%Our strategy to utilize these data will be presented based on their characteristics.
%In essence, we infer 
%
%We limit our demonstration to 6 main electron-impact processes of argon plasma (elastic momentum-transfer, direct ionization and 4 $1s$-level direct excitations);
%however, application to other collision processes must be straightforward.

==> sections-orig/model.tex <==
\section{Semi-empirical cross section models}\label{sec:model}

%\subsubsection{Employing semi-empirical models for the cross sections}
We observe from Figure~\ref{fig:crs-curation} that, for the most part,
the cross sections vary smoothly in $\epsilon$-space.
%All cross sections seem to vary smoothly over a certain $\epsilon$ range,
%implying a large correlation length.
Thus, while their reported measurement errors might be assumed
independent, this assumption certainly does not hold true for the
cross section itself.  Further, it suggests that the cross section
behavior can be adequately described with a low-dimensional parameter
set.
\par
%In order to capture the correlation in $\epsilon$-space,
To take advantage of this behavior,
we represent the cross sections $\sigma(\epsilon)$ with semi-empirical models $f(\epsilon;\vec{A})$, where $\vec{A}$ denotes the parameters of the model.
The parametric uncertainty for $\vec{A}$ represents the uncertainty of the cross section.
The semi-empirical models are based on theoretical arguments combined with a few empirical factors~\cite{Gargioni2008,Haddad1982,Bretagne1986,Kim1994}.
These model forms are intended to capture the essential features of the cross section using a
a relatively low-dimensional set of uncertain parameters.
%% SWC: original text for introduction of section 3.
%the cross section function is represented by semi-empirical formula with some model parameters,
%whose parametric uncertainty represents the uncertainty of the cross section.
%The semi-empirical models are based on theoretical estimations combined with a few empirical factors,
%to capture only the essential features for the plasma transport and chemistry.
%These semi-empirical cross section models will be introduced in Section~\ref{sec:model}.
\par
While some cross sections---excitations in particular---exhibit rich
fine-scale structures~\cite{Buckman1983, Zatsarinny2013}, most
datasets do not have the resolution necessary to support inference of
these features.  Further, the plasma transport and reaction properties
that are the primary quantities of interest in this work are integrals
over energy, and are therefore insensitive to these fine features in
the cross sections.  This insensitivity is demonstrated via
sensitivity analysis in \ref{app:sensitivity}. Thus, even when some
small-scale features are present---and thus a richer model would be
necessary to capture these features---we rely upon low-dimensional,
semi-empirical models.


%% SWC: original text for introduction of section 3.
%We represent the cross sections $\sigma(\epsilon)$, where $\epsilon$ denotes energy, with semi-empirical models $f(\epsilon;\vec{A})$, where $\vec{A}$ denotes the parameters of the model.
%These model forms are intended to capture essential features
%for reaction and transport with a relatively low-dimensional set of uncertain parameters~\cite{Gargioni2008,Haddad1982,Bretagne1986,Kim1994}.
%The cross section uncertainties, with measurement data $\mathcal{M}$, are then approximated with their parametric uncertainties $P(\vec{A} \vert \mathcal{M})$.

\subsection{Elastic momentum-transfer}\label{subsec:model-elastic}
For low electron-impact energy ($<1eV$),
the modified effective range theory (MERT) model has been widely used for the elastic momentum-transfer cross section~\cite{OMalley1963, Milloy1977, Haddad1982}.
The cross section is expressed as partial wave expansions,
\begin{subequations}\label{eq:mert}
\begin{equation}
f_{MERT}(\epsilon; \vec{A}_{MERT}) = \frac{4\pi}{k^2} \sum_{L=0}^{\infty} \sin^2(\eta_L - \eta_{L+1}),
\end{equation}
where $k^2 = (2m_e/\hbar^2)\epsilon$ with the electron mass $m_e$ and the reduced Planck constant $\hbar$.
The MERT formula determines the electron-atom scattering phase shift $\eta_L$ with 4 empirical factors $\vec{A}_{MERT} = \{A, D, F, \epsilon_1\}$,
\begin{equation}
k^{-1}\tan\eta_0 = -A\left[ 1 + \frac{4\alpha}{3a_0}k^2\log(ka_0) \right]
- \frac{\pi\alpha}{3a_0}k^2 + D k^3 + F k^4,
\end{equation}
\begin{equation}
k^{-1}\tan\eta_1 = \frac{\pi}{15}\alpha k\left(1 - \sqrt{\frac{\epsilon}{\epsilon_1}}\right)
\end{equation}
\begin{equation}
k^{-1}\tan\eta_L = \frac{\pi\alpha k}{(2L+3)(2L+1)(2L-1)a_0}
\qquad \text{for } L>1,
\end{equation}
\end{subequations}
with $a_0=5.29177\times10^{-11}m$ the Bohr radius and $\alpha = 11.08a_0^3$ the static polarizability of argon atom.
\begin{figure}
\centering
\input{figures/figure4.tex}
\caption{
The semi-empirical model (\ref{eq:mert-shift}) for the elastic momentum-transfer cross section,
together with the electron-beam experiment datasets.
The MERT model (\ref{eq:mert}) by Haddad and O'Malley~\cite{Haddad1982} is also included for a reference.
}
\label{fig:elastic-model}
\end{figure}
Figure~\ref{fig:elastic-model} shows the MERT model calibrated by Haddad and O'Malley~\cite{Haddad1982},
which agrees well with BSR calculation up to $1 eV$ and deviates from the electron-beam experiment data for the larger energy range.
\par
We note that, while the MERT model deviates for $>1eV$,
it exhibits a qualitatively similar trend with the electron-beam data,
and that it only requires a minor shift along $\epsilon$-axis.
Thus we designed an extension to the MERT model,
\begin{subequations}\label{eq:mert-shift}
\begin{equation}
f_{el}(\epsilon; \vec{A}_{el}) = f_{MERT}(\tilde{\epsilon}; \vec{A}_{MERT}),
\end{equation}
where $\vec{A}_{el}=\{\vec{A}_{MERT}, t_1, t_2, t_3\}$ includes three additional parameters,
which are used to determine the shift factor applied to $\epsilon$,
\begin{equation}\label{eq:mert-shift-factor}
\tilde{\epsilon} = \epsilon\left[ \frac{1 + t_1}{2} - \frac{1 - t_1}{2} \tanh\left(\frac{\epsilon - t_2}{t_3}\right) \right].
\end{equation}
\end{subequations}
In essence, (\ref{eq:mert-shift-factor}) amplifies $\epsilon$ by a factor of $t_1$ if $\epsilon > t_2$.
Figure~\ref{fig:elastic-model} shows the model with $\vec{A}_m$ least-square-fitted against the BSR dataset,
which seems flexible enough to capture the overall trend of the momentum-transfer cross section.
This model approximates the high-energy ($>10eV$) range with only $\cO(\epsilon^{-1})$ asymptote,
neglecting smaller-scale variations.
However, a sensitivity analysis using a zero-dimensional Boltzmann solver (\texttt{BOLSIG+}~\cite{Hagelaar2005})
indicated that the resulting swarm parameters are insensitive to these variations (see \ref{app:sensitivity}).

\subsection{Ionization}
Kim and Rudd~\cite{Kim1994, Gargioni2008} suggested a simple empirical form for the total ionization cross section
based on the binary-encounter-dipole model,
\begin{equation}\label{eq:ion}
f_i(\epsilon; \vec{A}_i) = \frac{4\pi a_0^2}{\epsilon / \epsilon_i}\left[a\log\frac{\epsilon}{\epsilon_i} + b\left(1 - \frac{\epsilon_i}{\epsilon}\right) + c\frac{\log(\epsilon/\epsilon_i)}{\epsilon/\epsilon_i + 1}\right],
\end{equation}
with $\epsilon_i = 15.760eV$ the first ionization energy of argon and $\vec{A}_i = \{a, b, c\}$ the model parameters for $f_i$.
\begin{figure}
\centering
\input{figures/figure5.tex}
\caption{
The semi-empirical model (\ref{eq:ion}) for the total ionization cross section,
together with the electron-beam experiment datasets.
}
\label{fig:ion-model}
\end{figure}
Figure~\ref{fig:ion-model} shows the empirical model evaluated using least-squares-fitted parameters, compared with the electron-beam datasets.

\subsection{Excitation---metastables}
%\todo[inline]{Explanation for each term?}
For $1s_5$, $1s_3$ excitation cross sections,
we employ a semi-empirical model suggested by Bretagne \textit{et al.}~\cite{Bretagne1986},
\begin{equation}\label{eq:metastable}
f_{me}(\epsilon; \vec{A}_{me}) = \frac{4\pi a_0^2R}{\epsilon}b_{me}\left(1 - \frac{\epsilon_{me}}{\epsilon}\right)\left(2\epsilon\right)^{-\gamma_{me}},
\quad
me = 1s_5, 1s_3,
\end{equation}
with $R = 13.606eV$ the Rydberg energy,
$\epsilon_{1s5} = 11.548eV$, $\epsilon_{1s3} = 11.723eV$ the excitation energies for $1s_5$ and $1s_3$ levels, respectively,
and the model parameters $\vec{A}_{me} = \{b_{me}, \gamma_{me}\}$.
The first term in (\ref{eq:metastable}) corresponds to the large-energy asymptotic limit from Bethe-Born approximation,
while the last two terms are the empirical factors for the low-energy range.
\begin{figure}
\centering
\input{figures/figure6.tex}
\caption{
The semi-empirical model (\ref{eq:metastable}) for the (a) $1s_5$ and (b) $1s_3$ level excitation cross section,
together with the electron-beam experiment datasets.
}
\label{fig:metastable-model}
\end{figure}
Figure~\ref{fig:metastable-model} shows the models with the literature values from Bretagne \textit{et al.}~\cite{Bretagne1986}.
The trends agree well with the measurement data.
The model, of course, cannot capture the fine resonance structures~\cite{Buckman1983} and the small-scale behaviors for $\epsilon - \epsilon_0 < 10^{-1} eV$,
which are observed in the BSR dataset.
A small sensitivity analysis via \texttt{BOLSIG+}~\cite{Hagelaar2005}, however,
revealed that the plasma chemistry and transport properties are insensitive to these fine features (see \ref{app:sensitivity}).

\subsection{Excitation---resonances}
For resonance level excitations $1s_4$ and $1s_2$,
we employ a similar model to that from Bretagne \textit{et al.}~\cite{Bretagne1986} which accounts for the relativistic effect for electrons,
\begin{equation}\label{eq:resonance}
f_{r}(\epsilon; \vec{A}_r) = \frac{4\pi a_0^2R^2}{\epsilon}\frac{F_{0,r}}{\epsilon_r}\left[\log\left(\frac{\epsilon}{(1 - \beta^2)\epsilon_r}\right) - \beta^2\right]\exp\left[-\frac{\gamma_r}{1 + \epsilon/\epsilon_r}\right],
\quad
r = 1s_4, 1s_2,
\end{equation}
where $\beta = \sqrt{2\epsilon/m_ec^2}$ the relativistic factor with the electron mass $m_e$ and the speed of light $c$,
and the model parameters $\vec{A}_r = \{F_{0,r}, \gamma_r\}$.
The excitation energies $\epsilon_{1s4} = 11.624eV$ and $\epsilon_{1s2} = 11.828eV$ are chosen from the NIST atomic spectra database~\cite{Kramida2022}.
The difference of (\ref{eq:resonance}) from the model by Bretagne \textit{et al.}~\cite{Bretagne1986} is the last empirical factor,
which adjusts the low-energy behavior.
This adjustment is similar to the low-energy empirical factor suggested by Paretzke~\cite{Gargioni2008}.
\begin{figure}
\centering
\input{figures/figure7.tex}
\caption{
The semi-empirical model (\ref{eq:metastable}) for the (a) $1s_4$ and (b) $1s_2$ level excitation cross section,
together with the electron-beam experiment datasets.
}
\label{fig:resonance-model}
\end{figure}
Figure~\ref{fig:resonance-model} shows results using reference parameter values.
The qualitative trends agree well with the measurement data.
\par
%The semi-empirical models in this section effectively capture the essential features for corresponding cross sections
%into a low-dimensional parameter space,
%which is advantageous for uncertainty quantification.
%The parametric uncertainties of these models are evaluated subsequently.


==> sections-orig/result.tex <==
\section{The inferred cross section uncertainty}\label{sec:result}

The probabilistic models from Section~\ref{sec:bayes}
are first compared for $1s_3$ excitation cross section as an example,
and their implications are discussed.
Then the parametric uncertainties of all 6 cross sections are calibrated and presented.

\subsection{Comparison of the parametric posterior distributions}
The posterior distributions from Section~\ref{sec:bayes} are sampled using a standard Markov chain Monte Carlo (MCMC) algorithm implemented in the \texttt{emcee} package~\cite{Foreman-Mackey2013}.
For all posteriors, the total sample size exceeds at least 20 times the auto-correlation length, typically around 50 times,
in order to obtain enough effectively independent samples~\cite{Foreman-Mackey2013}.
\par
\begin{figure}
\centering
\input{figures/figure8.tex}
\caption{
Sample scatter plots of the posterior distributions based
on the measurement-uncertainty-only representation (Section~\ref{subsec:wrong-bayes-1}) for $1s_3$ excitation cross section:
(a) with individual datasets ($P_1[\vA\vert\cM_m]$ in Eq.~\ref{eq:wrong-bayes1-indiv})
and (b) with all datasets combined ($P_1[\vA \vert \cM]$ in Eq.~\ref{eq:wrong-bayes1-total}).
}
\label{fig:wrong-bayes1}
\end{figure}
To illustrate the implication of neglecting the systematic error,
all the posteriors described in Section~\ref{subsec:wrong-bayes-1} are evaluated for the $1s_3$ excitation cross section.
Figure~\ref{fig:wrong-bayes1}~(a) shows samples from the posteriors $P_1[\vA \vert \cM_m]$ (\ref{eq:wrong-bayes1-indiv})
obtained from individual datasets $\cM_m$.
The individual posteriors are scattered in $\vA$-space,
and mostly do not overlap with each other.
This again reflects the scattering among the cross section datasets in Figure~\ref{fig:crs-curation}~(e),
implying that there is a large uncertainty in the cross section model parameters.
When evaluated using all the datasets simultaneously, however,
the probability description in Section~\ref{subsec:wrong-bayes-1} cannot capture this uncertainty.
In Figure~\ref{fig:wrong-bayes1}~(b),
the overall posterior $P_1[\vA \vert \cM]$ (\ref{eq:wrong-bayes1-total}) is highly concentrated in a narrow region,
indicating a very low uncertainty in $\vA$.
This is obviously a misleading conclusion given the scatter among the individual datasets.
\par
This does not mean that the Bayesian inference is wrong.
It is mathematically consistent given the likelihoods (\ref{eq:wrong-bayes1-total-likelihood2}) and (\ref{eq:wrong-bayes1-total-likelihood1}).
From (\ref{eq:wrong-bayes1-total-likelihood2}), each dataset $\cM_m$ claims a different best value of $\vA$ with its own measurement error $\delta \vsig_m$.
The overall likelihood (\ref{eq:wrong-bayes1-total-likelihood1}), which is simply the product of the likelihood for each dataset, naturally leads to a concentration of the posterior probability around a value somewhere in the middle.
This unrealistic result reflects the fact that the problem statement (\ref{eq:wrong-bayes1-statement}) does not properly account for all sources of uncertainty in the likelihood formulation.
%With the measurement error $\delta \vsig$ being the only uncertain factor in (\ref{eq:wrong-bayes1-statement}),
%any deviation observed in the measurement is ascribed entirely to the measurement error,
%no matter how small such likelihood is.
%As a result,
%the resulting posterior is evaluated with zero possibility for any other errors,
%thus essentially no uncertainty about the best-fitting parameter value.
\par
\begin{figure}
\centering
\input{figures/figure9.tex}
\caption{
Sample scatter plots of the posterior distributions of $1s_3$ excitation cross section:
(a) $P_2[\vA \vert \cM]$ (\ref{eq:wrong-bayes2}) based on the internal parametric uncertainty represenation (Section~\ref{subsec:wrong-bayes-2})
and (b) $P_3[\vA \vert \cM]$ (\ref{eq:gp-bayes-margin-post}) based on the Gaussian process representation (Section~\ref{subsec:gp-bayes}).
In both figures, samples are colored according to their posterior probability.
}
\label{fig:wrong-bayes2}
\end{figure}
The uncertainty underlying the scattering among datasets
can be captured only when it is explicitly considered in the probabilistic description.
Figure~\ref{fig:wrong-bayes2} shows the posterior distributions evaluated with the systematic error models.
Whether as an additional parameter uncertainty or as a Gaussian process,
considering the possibility of the systematic error
significantly increases the uncertainty of $\vA$.
While both posteriors are peaked at similar parameter values,
their distributions have qualitatively different shapes.
In turn, each systematic error model leads to a different conclusion about the uncertainties of the cross section model parameters:
while, with $P_2$ (\ref{eq:wrong-bayes2}), we may conclude that the uncertainty in $(\gamma, b)$ follows a Gaussian distribution with the uncertainty in $\gamma$ more pronounced,
$P_3$ (\ref{eq:gp-bayes-margin-post}) rather seems to conclude that $b$ is more uncertain.
%While there are some differences in their peak values or shapes,
%both posteriors seem to be similarly spread along the $\vA$-space.
\par
\begin{figure}
\centering
\input{figures/figure10.tex}
\caption{
Marginal posterior distribution $P[\sigma(\epsilon) \vert \cM]$ for $1s_3$ excitation cross section with
(a) $P_1[\vA \vert \cM]$ (\ref{eq:wrong-bayes1-total}) based on the measurement-uncertainty-only representation (Section~\ref{subsec:wrong-bayes-1});
(b) $P_2[\vA \vert \cM]$ (\ref{eq:wrong-bayes2}) based on the internal parametric uncertainty represenation (Section~\ref{subsec:wrong-bayes-2});
and (c) $P_3[\vA \vert \cM]$ (\ref{eq:gp-bayes-margin-post}) based on the Gaussian process representation (Section~\ref{subsec:gp-bayes}).
Shaded areas indicate the $68\%$, $95\%$ and $99.7\%$ credibility intervals of the posterior distribution.
}
\label{fig:wrong-bayes2-marginal}
\end{figure}
The difference between the two systematic error models appears more drastically when the uncertainty of the cross section $\sigma(\epsilon)$ is considered.
Figure~\ref{fig:wrong-bayes2-marginal} shows the distribution of $\sigma(\epsilon)$ obtained by forward propagating each $P[\vA \vert \cM]$ through the parametric model compared to the calibration data.
Once again, the results from (\ref{eq:wrong-bayes1-total}) do not capture the systematic errors among datasets,
with the probability concentrated on almost a single line.
On the other hand,
while the Gaussian process model seems to properly capture the scattering among the datasets,
the resulting posterior from the internal parametric uncertainty model is overly uncertain about $\vA$,
with its credibility intervals exceeding way beyond the measurement datasets.
Moreover, considering the median value of the cross section in $\epsilon>10^2eV$,
the internal parametric uncertainty model deviates from the datasets compared to the Gaussian process model,
implying a slight miscalibration of the parameter value.
\par
\begin{figure}
\centering
\input{figures/figure9-1.tex}
\caption{
Sample scatter plots of the posterior distributions of $1s_3$ excitation cross section on log scale of $b$:
(a) the internal parametric uncertainty represenation $P_2[\vA \vert \cM]$ (Eq.~\ref{eq:wrong-bayes2} in Section~\ref{subsec:wrong-bayes-2})
and (b) the Gaussian process representation $P_3[\vA \vert \cM]$ (Eq.~\ref{eq:gp-bayes-margin-post} in Section~\ref{subsec:gp-bayes})
compared with the measurement-uncertainty-only representation of individual datasets
$P_1[\vA\vert\cM_m]$ (Eq.~\ref{eq:wrong-bayes1-indiv} in Section~\ref{subsec:wrong-bayes-1}).
Samples for both $P_2[\vA \vert \cM]$ and $P_3[\vA \vert \cM]$ are colored according to their posterior probability.
}
\label{fig:wrong-bayes2-log}
\end{figure}
%
A deeper analysis of the posterior distributions can expose
the flaw of the internal parametric model and explain the overstated uncertainty.
In Section~\ref{subsec:wrong-bayes-2},
the systematic error is modeled using a Gaussian on $\vA$ as shown in (\ref{eq:dA-model}),
without considering the actual shape of the cross section model $f(\epsilon; \vA)$.
The resulting posterior cannot exactly capture the correlation
which inherently exists between parameters given the cross section model and the datasets.
For the $1s_3$ excitation, due to the model definition (\ref{eq:metastable}),
the two parameters $\{b, \gamma\}$ should be nonlinearly correlated roughly along $\gamma \sim \log b$.
Figure~\ref{fig:wrong-bayes2-log} shows the individual posteriors in Figure~\ref{fig:wrong-bayes1} using a log scale for $b$,
which exhibits a clear correlation of $\gamma\sim\log b$.
$P_2[\vA \vert \cM]$ (\ref{eq:wrong-bayes2}),
which is a joint Gaussian over $(b, \gamma)$-space,
now looks completely distorted in Figure~\ref{fig:wrong-bayes2-log}~(a).
A significant portion of the distribution deviates from the parameter values that are inferred from the datasets,
which contributes to the biased and overstated uncertainty observed earlier.
%assuming that
%there is no model-form error, and that the discrepancy among the datasets has the same correlation as for the cross section model $f(\epsilon;\vA)$.
%Such a viewpoint leads to the overstated uncertainty of the cross section model in two ways.
%First,
%due to the assumption of no model-form error,
%the resulting joint posterior (\ref{eq:wrong-bayes2-joint-posterior}) has no other terms to reflect the errors that do not fit into the cross section model,
%except $P_2\left[ \cM_m \big| \vA_m, \vA, \vtheta \right]$.
%This term represents the goodness-of-fit for the cross section model;
%however, these errors cannot be resolved even with the best-fitting parameter values,
%thus lowering the overall likelihood of the cross section model.
%Second, the systematic uncertainty is considered only on the parameter $\vA$-space with (\ref{eq:dA-model}),
%without a view to the actual shape of the cross section model $f(\epsilon; \vA)$.
%On the one hand, it is true that different parameter values can be inferred from different datasets, as observed in Figure~\ref{fig:wrong-bayes1}.
%On the other hand, a long distance in the parameter space does not necessarily mean that the resulting cross sections $f(\epsilon; \vA)$ are different.
%For example of $1s_3$ excitation, due to the model definition (\ref{eq:metastable}),
%that two parameters $\{b, \gamma\}$ should be nonlinearly correlated roughly along $b\sim \log\gamma$.
%This was also observed for all individual datasets in Figure~\ref{fig:wrong-bayes1}.
%Along this direction, two significantly different parameter points still can have similar cross sections, having similar likelihoods.
%The systematic error model (\ref{eq:dA-model}), however, cannot take this into account, 
%since it does not consider the actual shape of the model at all.
%Rather, it biases toward the parameter points that do not fit the measurement data well,
%simply because they are at a similar distance in the parameter space.
%Due to these two reasons,
%the internal parametric uncertainty model in Section~\ref{subsec:wrong-bayes-2}
%leads to an uncertainty representation that is not only overstated but also unable to capture
%the intrinsic correlation that should arise from the model form.
\par
Of course, in this case, it may be possible to improve the uncertainty model (\ref{eq:dA-model}) by assuming it to be a joint Gaussian distribution over $(\log b, \gamma)$-space, instead of $(b, \gamma)$.
However, such an improvement is predicated upon prior knowledge of the cross section model and the appropriate resulting correlation between the model parameters.
Such prior information is often unavailable, particularly for more complex or higher-dimensional models where the implicit dependencies among the parameters are more difficult to understand and characterize.
\par
On the other hand,
the Gaussian-process model considers the systematic error on the measurement space $(\epsilon, \sigma)$ directly.
As a result, both the goodness-of-fit and the systematic error are evaluated together via (\ref{eq:gp-bayes-indiv-likelihood}), against the actual measurement data $\cM_m$.
The resulting posterior properly captures the intrinsic correlation between $b$ and $\gamma$ arising from the model,
without explicitly requiring prior information be built into the model form.
%% SWC: original text of discussion.
%This difference exposes the implication of two different perspectives toward the systematic error.
%Gaussian-process model allows a general form of the model inadequacy and the discrepancy among the datasets.
%On the other hand,
%the internal parametric uncertainty model strongly assumes
%that there is no model-form error, and that the discrepancy among the datasets also has the same correlation as for the cross section model $f(\epsilon;\vA)$.
%However, this is not true in reality,
%and a significant portion of the error cannot be fit into the model $f(\epsilon;\vA)$.
%Due to the incapability to calibrate such error into the parametric uncertainty,
%the resulting posterior becomes overly uncertain about the parameter $\vA$.
\par
\begin{figure}
\centering
\input{figures/figure11.tex}
\caption{
Marginal cross section uncertainty of 6 electron-impact argon collision cross sections,
with the Gaussian process representation (Eq.~\ref{eq:gp-bayes-margin-post} in Section~\ref{subsec:gp-bayes}).
Shaded areas indicate the $68\%$, $95\%$ and $99.7\%$ credibility intervals of the posterior distribution.
The measurement data are marked the same as in Figure~\ref{fig:crs-curation}.
}
\label{fig:gp-bayes-all}
\end{figure}
This comparison leads to a conclusion that, among three different perspectives,
the probabilistic description in Section~\ref{subsec:gp-bayes} with a Gaussian-process systematic error
most properly reflects the nature of the measurement data.
All the cross section uncertainties are thus calibrated with the posterior formulation (\ref{eq:gp-bayes-margin-post}) in Section~\ref{subsec:gp-bayes}.
Figure~\ref{fig:gp-bayes-all}
shows the marginal cross section posteriors for all 6 collision processes.
For all cross sections,
the scattering among the datasets is captured within the credibility intervals.
There are some data that lie outside the credibility intervals:
in Figure~\ref{fig:gp-bayes-all}~(a),
except some outliers between $95$--$99.7\%$ interval,
the elastic cross section samples lie closely around the median value
and do not capture the small variation in $\epsilon > 10 eV$;
and all the excitation cross sections in Figure~\ref{fig:gp-bayes-all}~(c--f)
do not capture the BSR data in $\epsilon - \epsilon_0 < 0.1 eV$.
These are, of course, expected results from the cross section models chosen for this uncertainty quantification because the models chosen in Section~\ref{sec:model} cannot represent these features.
%from the justification that these features are confirmed  to be insignificant for the plasma chemistry and transport properties.
Their parametric uncertainties, therefore, do not reflect any deviation which the models cannot capture,
rather ascribing it to the systematic error (including the model inadequacy).
However, the resulting parametric uncertainty is still able to encompass the uncertainty in the plasma chemistry and transport properties,
which will be shown subsequently.

\subsection{Validation with swarm-parameter experiments}

The calibrated parametric model for the 6 collision cross sections
are forward-propagated to the swarm parameters via \texttt{BOLSIG+}
and compared with the experimental data from Table~\ref{tab:swarm-parameter}.
For the forward propagation,
the swarm parameters are evaluated with 7200 samples from the posterior distributions of the model parameters.
For each sample,
the collision cross section models from Section~\ref{sec:model} are evaluated and then used as inputs in \texttt{BOLSIG+} simulations.
\texttt{BOLSIG+} simulations are run at both the default condition of $300K$~\cite{Pitchford2013},
and also at different background temperatures to match with the experiment conditions in Table~\ref{tab:swarm-parameter}.
\par
\begin{figure}
\input{figures/figure12.tex}
\caption{
The cross section uncertainty propagated unto the swarm parameters,
shown with 3 credibility intervals ($68\%$, $95\%$, and $99.7\%$):
(a) drift velocity,
(b) the ratio of longitudinal diffusivity to mobility,
(c) the ratio of transverse diffusivity to mobility, and
(d) the reduced ionization coefficient.
The measurement data are marked the same as in Figure~\ref{fig:swarm-parameter}.
}
\label{fig:uncertainty-swarm}
\end{figure}
\begin{figure}
\input{figures/figure13.tex}
\caption{
The cross section uncertainty propagated unto the swarm parameters,
shown with 3 credibility intervals ($68\%$, $95\%$, and $99.7\%$):
the reduced excitation coefficients to
(a) $1s_5$,
(b) $1s_4$,
(c) $1s_3$, and
(d) $1s_2$.
The measurement data are marked the same as in Figure~\ref{fig:swarm-parameter-ex}.
}
\label{fig:uncertainty-swarm-ex}
\end{figure}
%\todo[inline]{Maybe rearrange the sentences in this paragraph $\downarrow$.}
Figure~\ref{fig:uncertainty-swarm}~and~\ref{fig:uncertainty-swarm-ex}
show the propagated uncertainty in the swarm parameters,
compared with the experimental data from Figure~\ref{fig:swarm-parameter}~and~\ref{fig:swarm-parameter-ex}.
As for the swarm-analysis data in Figure~\ref{fig:swarm-parameter-ex},
the evaluation of the reduced excitation coefficients in Figure~\ref{fig:uncertainty-swarm-ex}
requires the direct excitation cross sections to higher levels,
which uncertainties are not considered in the scope of our study.
Instead, the nominal cross sections for $2p$-level excitations
are chosen from BSR dataset~\cite{BSR-data} and included in each sample set of cross sections.
\par
Most of the experimental data lie within $95\%$ credibility intervals of the cross section uncertainty.
As mentioned in Section~\ref{subsec:swarm-data},
in Figure~\ref{fig:uncertainty-swarm}~(d)
the data from Specht \textit{et al.}~\cite{Specht1980} deviates from the credibility intervals,
as their measurements include contributions from the metastable population.
For the transport properties and the reduced ionization coefficients in Figure~\ref{fig:uncertainty-swarm},
the impact of the cross section uncertainties was relatively small,
and the experimental data also did not exhibit a large discrepancy with each other.
On the other hand,
the cross section uncertainties have a more significant impact on the reduced excitation coefficients, as shown Figure~\ref{fig:uncertainty-swarm-ex}.
%Considering that the uncertainty of higher-level excitation is not included,
%This indicates that, for the $1s$-level excitation rates,
%the direct excitation cross sections are currently the dominant uncertain factors.


==> sections/intro_old.tex <==
\section{Introduction}

\todo[inline]{more citations in the paragraph below $\downarrow$?}
Identifying cross-sections of molecular collision processes is crucial for accurate prediction of plasma physics~\cite{Gargioni2008}.
Reaction rates of plasma chemistry and plasma transport properties are determined by these collision processes~\cite{Vlcek1989, Bultel2002, Kapper2011}.
Amongst all, electron-impact collisions are particularly important for non-equilibrium plasma~\cite{Pitchford2017}.
Electron-impact collisions determines the specific form of electron energy distribution function (EEDF)~\cite{Pitchford2013, Pitchford2017},
which further impacts plasma chemistry and transport.
%\todo[inline]{Limit the scope to argon plasma somewhere.}
\par
\todo[inline]{The paragraph below $\downarrow$ is written assuming that the importance of collision cross-section is established in the paragraph above $\uparrow$.}
Accurate identification of a cross-section does not mean presenting the absolutely true value,
which in fact we deem not accessible ever.
Nor does it mean simply presenting the best-fitting value that produces the best prediction for most plasma simulations.
There is always the lack of our knowledge about a cross-section,
and such ignorance must be reduced for the accurate identification of the cross-section.
Such reduction, of course, is predicated upon the evaluation of the ignorance in a quantitative way.
Uncertainty quantification (UQ), particularly the Bayesian inference, can provide a systematic framework for this.
Based on our prior knowledge and observations from the experiments,
the lack of our knowledge can be quantitatively evaluated as uncertainty in a probabilistic description.
Such uncertainty can also be utilized to analyze the impacts on higher-level predictions
where the cross-sections are used as model inputs.
Our goal is to develop a Bayesian inference process where the uncertainty of a cross-section
can be evaluated from various measurement datasets.
While there are a massive number of species and collisions,
we mainly use the datasets for 6 major electron-argon collision processes
to present our UQ process: elastic momentum-transfer, direct ionization, and direct excitation to 4 $1s$-levels.
The same framework can be similarly applied to any other collision processes.
\par
\todo[inline]{Paragraph $\downarrow$: how much details do we need?}
There have been significant efforts to identify the electron-impact cross sections of argon plasma.
These efforts are characterized in mainly two categories:
direct cross-section measurements and swarm-parameter analysis.
%These efforts are characterized in mainly two approaches:\todo{elaborate them more.}
%electron-beam experiments and swarm-parameter analysis.
In the first category,
the cross-sections are directly measured either by electron-beam experiments or by \textit{ab initio} calculations.
Electron-beam experiments measure the scattering of a mono-energetic electron beam,
providing differential cross sections at specific energies and angles.
Combined with optical techniques, they can also provide excitation cross sections.
Recent developments in numerical techniques for quantum physics also enabled direct calculation of the cross-sections based on first principle.
On the other hand, swarm-analysis infers cross sections from measurements of transport properties,
which are relatively easier to measure with more accuracy.
While electron energy distribution function (EEDF) should be inferred with several approximations and simplifications,
the swarm-analysis can provide absolute cross-sections for impact energies below $1 eV$.
Detailed reviews of cross section measurements are available~\cite{Gargioni2008, Pitchford2013, Pitchford2017}.
In Section~\ref{sec:curation}, we curate and categorize the measurement data for these cross sections into direct measurements and swarm-analysis.
\par
Thanks to such efforts, generic forms and values of electron-impact cross sections are well-known.
Their underlying uncertainties, however, have not been assessed well.
While electron-beam experiments provide direct cross-section measurements with explicitly reported accuracy,
these measurements involve systematic errors varying from experiments to experiments~\cite{Gargioni2008}.
Most of these biases are difficult to assess,
and as a result there are a large discrepancies among the datasets from electron-beam experiments, compared to their reported accuracies.
On the other hand,
despite accurate measurement of the transport properties,
the swarm-analysis relies upon the inference procedure with a simplified Boltzmann equation,
where a set of many collision processes interact with each other in an implicit and nonlinear way.
As a result, the dependence of the swarm parameters on the cross-sections cannot be expressed with a simple, explicit algebraic relation,
and likewise the uncertainty of the inferred cross-section remains implicit.
The correlation between the inferred cross-sections is also not well investigated for the same reason.
\par
Most reviews of cross-section datasets~\cite{Gargioni2008, Pitchford2013, Pitchford2017}
merely compare them and report their discrepancies.
Naively taking these discrepancies as uncertainties can be problematic,
since it would only represent a marginal probability at a single electron energy, entirely missing the correlation along the electron energy space.
Furthermore, these discrepancies can be misleading when the datasets are inter-dependent.
This is indeed the case for swarm-analysis datasets~\cite{Pitchford2013},
where it is often necessary to adopt cross sections from other sources, either for a certain energy range or for a collision process.
As a result, a small discrepancy among datasets is often due to sharing the same source, not necessarily representing a small uncertainty.
%\par
%One reason is because cross sections are often not directly measurable, even with electron-beam experiments.
%As a result, most experiments involve some inference procedures with assumptions.\todo{Elaborate more with examples.}
%Uncertainties underlying in this procedure are usually hard to be quantified,
%and the reported accuracies of the experiments are often notional.
%\par
%Another reason is the difficulty of identifying correlation along electron energy space.
%While a cross section must be a function of energy and thus cross section values at any energy points are dependent on each other,
%its true functional form is not known (and probably will never be).
%So it is necessary to 
\par
In this paper, we assess the cross-section uncertainties of the electron-argon collision processes under Bayesian framework.
Due to the implicit dependence of the swarm-parameter measurements on cross-sections,
it was decided to infer the cross-sections using only the electron-beam measurements
and reserve the swarm-analysis data for validation of the resulting model.
Details of this decision process will be discussed in Section~\ref{sec:curation}.
%The cross-sections $\sigma(\epsilon)$ were characterized using
Semi-empirical models with a few parameters are used to characterize the cross-sections~\cite{Gargioni2008,Haddad1982,Bretagne1986,Kim1994},
with an expectation that their parametric uncertainty would be sufficient to
capture the essential features of the cross-sections that are relevant to the plasma reaction and transport processes.
\par
Formulating a proper likelihood model is crucial to accurately assess the uncertainty underlying the data.
The parametric uncertainty, of course, is not the only source of the cross-section uncertainty.
Part of the error between the model and the data can be attributed to the inherent inadequacy of the cross-section model.
Furthermore, as described earlier, systematic errors of the experiments can also induce the discrepancies, even among the datasets.
This is particularly true for the electron-beam data,
where the discrepancy is significant and cannot be explained by their reported observation errors.
A naive likelihood that does not reflect these factors can lead us to a misleading conclusion about the underlying uncertainty of the cross-sections.
Here, the combined effects of this systematic error and any inherent inadequacy in the semi-empirical
cross section model is represented statistically using a Gaussian process~\cite{Kennedy2001}.
\par
In Section~\ref{sec:curation},
we summarize the curated data for the 6 collision processes, both for the direct measurement and the swarm-analysis.
In Section~\ref{sec:model},
the semi-empirical cross-section models chosen for the Bayesian inference are introduced.
In Section~\ref{sec:bayes},
the framework for the Bayesian inference is introduced,
and the likelihood and the posterior probability are formulated.
In Section~\ref{sec:result},
the inferred parametric uncertainty of the cross-sections are reported.
This is compared with the result of the naive likelihood,
demonstrating the importance of the systematic error modeling in the Bayesian framework.
The inferred uncertainties are then propagated using a 0-D Boltzmann solver,
and validated with the swarm-parameter data.
In Section~\ref{sec:conclusion},
we summarize our study and future works.

%The goal of this paper is to properly assess the cross-section uncertainties that are essential for the plasma reaction and transport processes.
%It is crucial to have a formulation that can quantitatively reflects our knowledge under statistical principles,
%and still can be evaluated in a computationally efficient manner.
%We employ a Bayesian approach to infer cross-section uncertainties from measurement data.
%Since the swarm parameters are indirectly determined by the cross sections and dependent on
%additional modeling choices, it was decided to infer the cross
%sections using only the direct measurements and reserve the swarm-analysis data for validation of the resulting model.
%The detailed decision process for this will be presented in Section~\ref{sec:curation}.
%\par
%The cross sections $\sigma(\epsilon)$ were characterized using
%semi-empirical models $f(\epsilon;\vec{A})$, where $\epsilon$ denotes
%energy and $\vec{A}$ represents the model
%parameters~\cite{Gargioni2008,Haddad1982,Bretagne1986,Kim1994}.  The
%motivation for this choice was the expectation that these models,
%coupled with their parametric uncertainty, would be sufficient to
%capture the essential features of the cross-sections that are relevant
%to the plasma reaction and transport processes.

%This is particularly true for
%
%
%The goal of this paper is to assess the uncertainties of the electron-impact collision cross sections that are crucial for
%under statistical principles.
%Since the swarm parameters are
%indirectly determined by the cross sections and dependent on
%additional modeling choices, it was decided to infer the cross
%sections using only the direct measurements and reserve the swarm
%parameter data for validation of the resulting model.
%
%
%Our strategy to utilize these data will be presented based on their characteristics.
%In essence, we infer 
%
%We limit our demonstration to 6 main electron-impact processes of argon plasma (elastic momentum-transfer, direct ionization and 4 $1s$-level direct excitations);
%however, application to other collision processes must be straightforward.
